Chameleon: Plug-and-Play Compositional Reasoning with Large Language Models

Large language models (LLMs) have achieved remarkable progress in solving various natural language processing tasks due to emergent reasoning abilities. However, LLMs have inherent limitations as they are incapable of accessing up-to-date information (stored on the Web or in task-specific knowledge bases), using external tools, and performing precise mathematical and logical reasoning. In this paper, we present Chameleon, an AI system that mitigates these limitations by augmenting LLMs with plug-and-play modules for compositional reasoning. Chameleon synthesizes programs by composing various tools (e.g., LLMs, off-the-shelf vision models, web search engines, Python functions, and heuristic-based modules) for accomplishing complex reasoning tasks. At the heart of Chameleon is an LLM-based planner that assembles a sequence of tools to execute to generate the final response. We showcase the effectiveness of Chameleon on two multi-modal knowledge-intensive reasoning tasks: ScienceQA and TabMWP. Chameleon, powered by GPT-4, achieves an 86.54% overall accuracy on ScienceQA, improving the best published few-shot result by 11.37%. On TabMWP, GPT-4-powered Chameleon improves the accuracy by 17.0%, lifting the state of the art to 98.78%. Our analysis also shows that the GPT-4-powered planner exhibits more consistent and rational tool selection via inferring potential constraints from instructions, compared to a ChatGPT-powered planner. The project is available at https://chameleon-llm.github.io.

==> codes/algoritm.tex <==

\begin{algorithm}[t!]
\caption{Dynamic Prompt Learning via Policy Gradient (\model)}
\label{alg:policy}
\small
\hspace*{0.02in} {\bf Input:} 
 Initial policy $\pi_{\theta_0}$, training example set $P_{\text{train}}$, candidate example set $E_{\text{cand}}$, \# of training epochs $N$ \\
\hspace*{0.02in} {\bf Output:}
Learned policy $\pi_\theta$
\begin{algorithmic}[1]
    \Function{REINFORCE}{$\pi_{\theta_0}$, $P_{\text{train}}$, $E_{\text{cand}}$, $N$}
        \State Initialize policy network $\pi$ with parameter $\theta_0$
        \For{epoch = $1,2,...,N$}
        \For{$P_{\text{batch}} \in P_{\text{train}}$} \Comment{get a batch from the training set}
        \State $\mathcal{L}_{\text{batch}} \gets 0$
        \For{$p_i \in P_{\text{batch}}$}
            \State Sample  $e_i^k \sim \pi_{\theta}(e_i | p_i), e_i^k \in E_{\text{cand}}, k=\{1,...,K\}$ \Comment{$K$ is \# of in-context examples}
            \State $\hat{a}_i \gets \text{GPT-3}(e_i^1,...,e_i^k, p_i)$ \Comment{$\hat{a}_i$ is the GPT-3 generated answer}
            \State $r_i \gets \text{\scshape Eval}(\hat{a}_i, a_i), r_i \in \{-1, 1\}$ \Comment{$a_i$ is the ground truth answer of $p_i$}
            \State $\mathcal{L}_{\text{batch}} \gets \mathcal{L}_{\text{batch}} - r_i \cdot \ln \pi_{\theta}(e_i | p_i)$
        \EndFor
        \State Optimize $\mathcal{L}_{\text{batch}}$ wrt. $\theta$
        \EndFor
        \EndFor
        \State \Return $\pi_{\theta}$
    \EndFunction
\end{algorithmic}
\label{algorithm}
\end{algorithm}

==> tables/tool_num.tex <==

\begin{figure*}[t!] 
 \centering
 % \renewcommand\tabcolsep{4.0pt} % column space
 % \renewcommand\arraystretch{1.1} % row space
 % \resizebox{1.0\linewidth}{!}{
 \begin{tabular}{llcc} 
 \toprule
 \header{Task} & \header{Model} & \header{\# of different programs} & \header{Average program length} \\
 \midrule
 \multirow{3}{*}{\scienceqa} & CoT  & 1 & 2 \\
 & \modelchatgpt & 14 & 3.03 \\
 & \modelgpt & 11 & 3.40 \\
 \midrule 
 \multirow{4}{*}{\tabmwp} & CoT & 1 & 2 \\
 & PoT & 1 & 2 \\
 & \modelchatgpt & 28 & 4.17 \\
 &\modelgpt  & 19 & 4.09 \\
 \bottomrule
 \end{tabular}
 % }
 \captionof{table}{The statistics of the number of different generated programs and the average length of generated programs by our \model, respectively. Chain-of-thought (CoT) prompting and Program-of-thought (PoT) prompting are also compared as they are the special cases of \model.}
 \label{tab:tool_num}
\end{figure*}


==> v1_arxiv_backup/appx.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hrule height 4pt
% \vskip 0.25in
% \vskip -\parskip
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \fontsize{24pt}{\baselineskip}\selectfont {
% % Supplementary Materials for \\ \hspace*{\fill} \\ IconQA: A New Benchmark for Abstract Diagram Understanding and Visual Language Reasoning}
% \vbox{
%     \centering
%     \LARGE 
%     \textbf{Supplementary Materials for \\  
%     LLM}
% }
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vskip 0.29in
% \vskip -\parskip
% \hrule height 1pt
% \vskip 0.09in
% % \vskip 0.15in
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \renewcommand*\footnoterule{} % remove the separator line

% \newcommand\blfootnote[1]{%
%   \begingroup
%   \renewcommand\thefootnote{}\footnote{#1}%
%   \addtocounter{footnote}{-1}%
%   \endgroup
% }

% \blfootnote{
%     \footnotesize 
%     \\36th Conference on Neural Information Processing Systems (NeurIPS 2022).
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Appendix}
\label{app}

% This appendix includes
% \begin{itemize}
%     \item Implementation details including the planner policy and module configurations (Sec. \ref{app:exp_details})
%     \item More qualitative results on \scienceqa (Sec. \ref{app:case_study_scienceqa})
%     \item More qualitative results on \tabmwp (Sec. \ref{app:case_study_tabmwp})
%     % more  qualitative  results
% \end{itemize}



% \subsection{Experimental Details}
% \label{app:exp_details}

\input{tables/policy_scienceqa}

\input{tables/policy_tabmwp}


\input{tables/policy_tools}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/sqa-gpt4.pdf}
    \caption{Transitions between modules in programs generated by \model (GPT-4) on \scienceqa.  START is the start symbol, END is a terminal symbol and the others are non-terminal symbols.}
    \label{tab:transition_scienceqa}
\end{figure*}


\begin{figure*}[ht!]
    \centering
    \includegraphics[width=0.85\linewidth]{figs/tabmwp-gpt4.pdf}
    \caption{Transitions between modules in programs generated by \model (GPT-4) on \tabmwp. START is the start symbol, END is a terminal symbol and the others are non-terminal symbols.}
    \label{tab:transition_tabmwp}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/showcase_scienceqa_more.pdf}
    \caption{One example from our \model (GPT-4) on \scienceqa.}
    \label{fig:showcase_scienceqa_more}
\end{figure*}

% \subsection{Case Study: \scienceqa}
% \label{app:case_study_scienceqa}

% \subsection{Case Study: \tabmwp}
% \label{app:case_study_tabmwp}




==> v1_arxiv_backup/body.tex <==
%%%%%%%%% BODY TEXT

\section{Introduction}
\label{sec:intro}
% \pan{Recent progress of large language models, especially in the field of reasoning}

Remarkable progress has been observed in recent large language models (LLMs) for various natural language processing tasks, with prominent examples such as GPT-3 \cite{brown2020language}, PaLM \cite{chowdhery2022palm}, LLaMA \cite{llamaadapter2023}, ChatGPT \cite{openai2022chatgpt}, and the more recently proposed GPT-4 \cite{OpenAI2023GPT4TR}. LLMs have demonstrated emergent abilities, including in-context learning, mathematical reasoning, and commonsense reasoning \cite{wei2022emergent}. These models are capable of solving diverse tasks in a zero-shot fashion \cite{kojima2022large} or with the aid of a few examples \cite{wei2022chain}, and they show great potential in planning and decision-making akin to human beings \cite{huanginner2022}. However, LLMs have inherent limitations, such as an inability to access up-to-date information \cite{komeili2022internet}, utilize external tools \cite{schick2023toolformer}, or perform precise mathematical reasoning \cite{patel2021nlp, lu2022dl4math}.

% \pan{Recent attempts in tool use, analysis of the limitations of current work}

To address these limitations of LLMs, an active research direction involves augmenting language models with access to external tools and resources, as well as exploring the integration of external tools and plug-and-play modular approaches. For example, aided by web search engines and  external knowledge resources, LLMs are able to access real-time information and leverage
domain-specific knowledge \cite{nakano2021webgpt}. To enhance mathematical reasoning abilities, recent work uses LLMs \cite{chen2021evaluating} to generate complex programs to exploit powerful computational resources, and execute logical reasoning tasks more effectively \cite{wang2022code4struct,gao2022pal,chen2022program,mishra2022lila,imani2023mathprompter,paranjape2023art}. Another line of recent work, such as ViperGPT \cite{suris2023vipergpt}, Visual ChatGPT \cite{wu2023visual}, VisProg \cite{gupta2022visual}, and HuggingGPT \cite{shen2023hugginggpt} incorporates a collection of foundation computer vision models to equip LLMs with the abilities to perform visual reasoning tasks.

Despite significant progress, current tool-augmented LLMs still face critical challenges when addressing real-world queries. Most existing approaches are either limited to a small number of tools \cite{mishra2022lila,chen2022program,wang2022code4struct,imani2023mathprompter,paranjape2023art,schick2023toolformer} or rely on domain-specific tools \cite{nakano2021webgpt,yang2023mm,gupta2022visual,wu2023visual,suris2023vipergpt}, and thus are not easy to generalize to diverse queries. Consider the example in \autoref{fig:showcase_scienceqa}: \textit{Which is the main persuasive appeal used in this ad?}. To answer this question, one needs to: 1) infer that there is an ad image containing text context and call a text decoder to understand the semantics; 2) retrieve background knowledge to clarify the definition of \textit{persuasive appeal} and the differences among various types; 3) generate a solution based on the clues from the input query and intermediate results from previous steps; and 4) finally produce the answer in a task-specific format. On the other hand, when answering \textit{Which animal's skin is adapted for survival in cold places}, one might need to call other modules, such as an image captioner to decipher image information and a web search engine to retrieve domain knowledge to understand scientific terminologies.

To address these challenges, we introduce~\model, a \textit{plug-and-play compositional} reasoning framework that harnesses the capabilities of large language models.~\model~is capable of synthesizing programs to compose various tools to tackle a broad range of queries. 
While it does not require any training, \model uses the in-context learning capabilities of LLMs to generate these programs.
In contrast with existing approaches \cite{schick2023toolformer, nakano2021webgpt,yang2023mm,gupta2022visual,wu2023visual,suris2023vipergpt}, it employs diverse types of tools, including LLMs, off-the-shelf computer vision models, web search engines, Python functions, and rule-based modules tailored to specifically customized tasks.~\model~builds on top of an LLM as a natural language planner. Prompted by descriptions of each tool and examples of tool usage, the planner can infer an appropriate sequence of tools to compose and execute in order to generate the final response for a user query. Unlike previous work that generates domain-specific programs \cite{nakano2021webgpt, suris2023vipergpt, gupta2022visual}, \model generates natural-language-like programs, which are less error-prone, easy to debug, user-friendly for those with limited programming experience, and efficiently extendable to using new modules. During the execution of each module in the program, the module processes the query and caches context, returns a result determined by the module itself, and updates the query and cached context for subsequent module execution. Composing modules as a sequential program, the execution of subsequent modules can leverage the prior cached context and updated queries.

We showcase the adaptability and effectiveness of \model on two tasks: \scienceqa \cite{lu2022learn} and \tabmwp \cite{lu2023dynamic}. \scienceqa is a multi-modal question answering benchmark spanning multiple context formats and various scientific topics, while \tabmwp is a mathematical benchmark involving diverse tabular contexts. These two benchmarks serve as a good testbed to evaluate \model's ability to coordinate diverse tools across different types and domains. Notably, \model with GPT-4 achieves an 86.54\% accuracy on \scienceqa, significantly improving upon the best published few-shot model by 11.37\%. On \tabmwp, using GPT-4 as the underlying LLM, \model achieves an improvement of 7.97\% over CoT GPT-4 and a 17.8\% increase over the state-of-the-art model, leading to a 98.78\% overall accuracy on \tabmwp. Further studies suggest that using GPT-4 as a planner exhibits more consistent and rational tool selection and is able to infer potential constraints given the instructions, compared to other LLMs like ChatGPT.

% \model built upon ChatGPT attains an accuracy of 93.28\%, an improvement of 11.25\% over the chain-of-thought (CoT) prompted ChatGPT. When 
% \pan{Differentiate our work?}

% (1) \textit{cross-task generalization}

% (2)\textit{ Easy to debug}

% (3) \textit{interpretable}

% (4) et al

% \red{We introduce V
% ISP
% ROG which inputs visual data (a sin- gle image or a set of images) along with a natural language instruction,  generates  a  sequence  of  steps,  a visual  pro- gram if you will, and then executes these steps to produce the desired output}

% \red{Modules may be off-the-shelf computer vi-
% sion  models,  language  models,  image  processing  subrou- tines  in  OpenCV  [4],  or  arithmetic  and  logical  operators.}

% Auto-GPT

% \pan{Summarize our contributions}
In summary, our contributions are as follows:
(1) We develop a plug-and-play compositional reasoning framework, \model, that effectively leverages large language models to address their inherent limitations and tackle a broad range of reasoning tasks. (2) We successfully integrate various tools, including LLMs, off-the-shelf vision models, web search engines, Python functions, and rule-based modules, to build a versatile and adaptable AI system to answer real-world queries. (3) We showcase the framework's adaptability and effectiveness on two challenging benchmarks, \scienceqa and \tabmwp, significantly improving the state of the art.
%results. achieving significant improvement over the best published few-shot results.



\section{Related Work}
\label{sec:related}
\subsection{Large Language Models}

In recent years, the development of large language models (LLMs) has made tremendous progress, as evidenced by models such as BLOOM \cite{scao2022bloom}, PaLM \cite{chowdhery2022palm}, Flan-T5 \cite{chung2022scaling}, LLaMA \cite{touvron2023llama}, GPT-3 \cite{brown2020language}, ChatGPT \cite{openai2022chatgpt}, and GPT-4 \cite{OpenAI2023GPT4TR}. These LLMs exhibit emergent abilities, including in-context learning, mathematical reasoning, and commonsense reasoning. LLMs like GPT-3 and GPT-4 are capable of solving various tasks using zero or only a handful of task-relevant examples. The chain-of-thought (CoT) approach \cite{wei2022chain} instructs LLMs to decompose complex problems by generating intermediate reasoning steps before arriving at the final answer. Another active research area is to incorporate external verification \cite{peng2023check,madaan2023self} and human feedback \cite{openai2022chatgpt} to allow LLMs to perform more reliably and align better with human preferences. In addition, a recent line of work focuses on instruction learning, either via generating high-quality instructions data \cite{peng2023instruction} or by boosting the language models with instructions, such as Flan-T5 \cite{chung2022scaling}, LLaMA \cite{touvron2023llama}, LLaMA-Adapter \cite{llamaadapter2023}, and LLaVA \cite{liu2023llava}. Our proposed~\model~builds on these lines of work, introducing a general approach that enables cross-task generalization, leverages in-context learning from demonstrations, and integrates various capabilities of external tools to solve complex reasoning problems. 

\subsection{Compositional Reasoning}

Neural modular and compositional approaches have been explored to automatically perform desired sub-task decomposition, enhancing interpretability and adaptability across various reasoning tasks. Early work \cite{andreas2016learning, andreas2016neural} posits that complex reasoning tasks are fundamentally compositional and proposes neural module networks (NMN) to decompose them into subtasks. However, these methods rely on brittle off-the-shelf parsers and are limited by module configurations. Some later work \cite{johnson2017inferring,hu2017learning,hu2018explainable} takes a step further by predicting instance-specific network layouts in an end-to-end manner, without relying on parsers, using reinforcement learning \cite{williams1992simple} and weak supervised learning. % answer supervision. 
In visual reasoning, models comprising a program generator and an execution engine have been proposed to combine deep representation learning and symbolic program execution \cite{johnson2017inferring, yi2018neural}. In the domain of mathematical reasoning, an interpretable problem solver has been developed to incorporate theorem knowledge as conditional rules and perform symbolic reasoning step by step \cite{lu2021inter}.

Our work takes inspiration from neural module networks, yet it offers several distinct advantages. First,~\model~does not require expensive supervision in the form of task-specific programs. Instead, it generates sequential programs, consisting of modules, that are easy to generalize to various domains and tasks, allowing for the extension to new modules in a plug-and-play manner. Second,~\model~does not require any training, but uses the in-context learning capabilities of LLMs to generate programs prompted by natural language instruction and demonstrations.


\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/showcase_tabmwp_long.pdf}
    \caption{Three examples from our~\model~with GPT-4 on \tabmwp \cite{lu2023dynamic}, a mathematical reasoning benchmark with tabular contexts. \model demonstrates flexibility and efficiency in adapting to different queries that require various reasoning abilities.}
    \label{fig:showcase_tabmwp}
    % \vspace{-2mm}
\end{figure}


\input{tables/comparison}

\subsection{Tool-Augmented Language Models}
Despite impressive performance of LLMs, %\cite{brown2020language,openai2022chatgpt} and demonstrate emergent capabilities \cite{wei2022emergent} across various natural language processing tasks. However, these language models also 
they suffer from inherent limitations, such as the inability to access up-to-date information \cite{komeili2022internet}, utilize external tools \cite{schick2023toolformer}, or perform precise mathematical reasoning \cite{patel2021nlp, lu2022dl4math}. To address these shortcomings, there has been a growing interest in exploring the use of external tools and modular approaches to augment LLMs. These augmented LLMs can access real-time information aided by web search engines \cite{nakano2021webgpt} and leverage domain-specific knowledge from external resources \cite{yu2023generate}.  Some work leverages the Python interpreter to generate complex programs to employ powerful computational resources, and execute logical reasoning tasks more effectively \cite{wang2022code4struct,gao2022pal,chen2022program,mishra2022lila,imani2023mathprompter,paranjape2023art}.
For example, Toolformer \cite{schick2023toolformer} constructs tool-use augmented data to train language models to select five tools. In the realm of visual tools, various approaches have been proposed to enhance the capabilities of large language models in handling visual tasks \cite{yang2023mm,wu2023visual,suris2023vipergpt,gupta2022visual,shen2023hugginggpt}, augmented with Hugging Face models \cite{shen2023hugginggpt}, Azure models \cite{yang2023mm}, visual foundation models \cite{wu2023visual}.

We compare~\model~with other tool-augmented language models in \autoref{tab:tool_comparison}. Many of these approaches are either constrained to a small set of tools or limited to task-specific tools, which reduces their capabilities across various skill dimensions and hampers their generalizability to new tasks. A recent line of work relies on large amounts of supervision \cite{schick2023toolformer, komeili2022internet} and focuses on generating commands \cite{nakano2021webgpt} and programs \cite{suris2023vipergpt,gupta2022visual} to infer the choice of tools. However, this approach needs to carefully tailor prompts to specific tasks and particular tools, and is neither flexible nor adaptive. 
%potentially hindering its flexibility and adaptability. 
In contrast,~\model~instructs LLMs with natural language instructions that simply describe the roles of each rule and provide a few calling examples, eliminating the need for additional training or tool-specific prompts when learning to compose different tools. More importantly,~\model~offers users flexibility in terms of tool types and sources, updating the underlying LLMs, adding new tools, and adapting to new tasks by updating the instructions. Our work shares the same spirit of AutoGPT \cite{autogpt2023}, an autonomous GPT-4 agent with the artificial general  intelligence (AGI) ambition to incorporate numerous tools to achieve user-defined goals. While AutoGPT is still under development, our work is the first to instantiate the idea and verify its effectiveness on well-studied benchmarks.




\section{General Framework:~\model}

Distinct from previous approaches, our~\model~method is capable of synthesizing the composition of various tools to accommodate a wide range of problems. It employs a natural language planner, $\cP$, to generate a sequential program to select and compose modules stored in an inventory, $\mathcal{M}$. Then, the program is executed 
%the modules are bound and executed sequentially 
to generate the answer. 
%\model~ enabling a flexible and adaptive problem-solving process.

% \subsection{Natural Language Planner}
% \pan{module definition, one example}
% \pan{Apply the terminology of program synthesis to introduce our method.}
%Here, we only provide a high-level description of our planner, and leave more implementation details (e.g., prompts) to later sections.
We formalize our planner as follows:
given the input query $x_0$, the module inventory $\mathcal{M}$, and constraints $\cG$, the natural language planner $\cP$ selects a set of modules that can be executed sequentially to solve the problem. 
In our work, the planner $\cP$ is an LLM prompted to generate a sequence of module names in a few-shot setup (see details in the appendix). 
The module inventory $\mathcal{M}$ consists of a set of pre-built modules: $\{M_i\}$, each corresponding to a tool of various types (\autoref{fig:tools}).
%, , e.g., OpenAI models, Hugging Face models, GitHub models, search engines, Python interpreters, and rule-based functions.
A $T$-lengthed plan sampled from $\cP$ is denoted as $p = {M^1, \dots, M^T}$, where $M^t\in\mathcal{M}$. Formally, a plan $p$ is generated as follows:
\begin{equation}
    p \leftarrow \cP (x_0; \cM; \cG),
\end{equation}
where $\cG$ are the constraints for the plan generation, and $x_0$ the input query (problem statement). 
%
Given the generated plan, the corresponding modules for each step are then executed sequentially. When evaluating the module $M^t$ at time step $t$, the output of the execution $y^t$ is calculated by:
\begin{equation}
 y^t \leftarrow M^t (x^{t-1}; c^{t-1}),
\end{equation}
where $x^{t-1}$ is the input for the current module $M^t$, and $c^{t-1}$ is the cached information gathered from the history modules.

Both the problem input $x^t$ and cache $c^t$ for the next module $M^{t+1}$ are updated, respectively, by:
\begin{equation}
\begin{aligned}
 x^t &\leftarrow \texttt {update\_input}(x^{t-1}, y^t), \\
 c^t &\leftarrow \texttt {update\_cache}(c^{t-1}, y^t).
\end{aligned}
\end{equation}

Finally, the answer $a$ to the problem is generated by the last module $M^T$:
\begin{equation}
 a = y^T\leftarrow M^T (x^{T-1}; c^{T-1}).
\end{equation}

% \input{codes/algoritm}

\begin{table*}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/tools.pdf}
    \caption{Different types of tools in our module inventory.}
    \label{fig:tools}
    % \vspace{-10mm}
\end{table*}




\section{Applications of \model}

We demonstrate the applications of \model on two challenging reasoning tasks: ScienceQA \cite{lu2022learn} and TabMWP \cite{lu2023dynamic}. The module inventory is introduced in \autoref{sec:module}, and the specific designs for these two tasks are presented in \autoref{sec:sqa} and \autoref{sec:tabmwp}, respectively.


\subsection{Module Inventory}
\label{sec:module}

% \pan{Introduce the modular sets. List all the modules}


To accommodate various problem-solving capabilities over a diverse range of problems, it is necessary for our system to leverage a rich module inventory containing various external tools. 
In this section, we give a high-level description of the module inventory we used and defer the descriptions of detailed implementations to specific experiments.
The complete module inventory, denoted as $\mathcal{M}$, is presented in \autoref{fig:tools}. Each tool within the inventory is defined as follows:

\textbf{Knowledge Retrieval} ($M_{kr}$): Retrieving extra background knowledge is crucial for assisting the system in tackling complex problems. Here, the ``Knowledge Retrieval'' module is designed to obtain domain-specific knowledge in a generative manner, i.e., prompting the LLMs to generate relevant background information for the given query, as done by \cite{suris2023vipergpt}. Typically, this module is beneficial for providing useful task contexts for solving problems from specialized domains, such as science and mathematics. For instance, if a question is about a tax form table, this module could generate knowledge pertaining to tax procedures, providing valuable context for the task at hand.
% tax regulations and procedures

\textbf{Bing Search} ({$M_{bs}$}): Similar to the generative ``Knowledge Retrieval'', the goal of the ``Bing Search'' here is to provide broader coverage of task-relevant knowledge. In contrast to the generative ``Knowledge Retrieval'' module, the ``Bing Search'' module demonstrates its strengths in cases where a broader range of information is needed or the query requires up-to-date information from multiple sources. We implement this module using the search engine API to return relevant search results based on the input query. The returned results can then be parsed and utilized by other modules within the system to gather richer context information from diverse sources to support problem-solving more effectively.


\textbf{Query Generator} ($M_{qg}$): Generally, the original problem does not contain any tailored query for retrieving task-relevant information from the search engine. Thus, the query generator is designed to create search engine queries based on the given problem, which is then used as inputs to the ``Bing Search'' module. 
For most cases, it is a good strategy to use the ``Query Generator'' module before the ``Bing Search''. In other words, coupled with the search engine tool, generating more targeted queries generally facilitates both the recall and precision of retrieved information. 

\textbf{Image Captioner} ($M_{ic}$): This module is designed to generate captions for images, which can be employed to offer additional context for the given question. Typically, the ``Image Captioner'' is utilized when a question requires a semantic understanding of an image. By leveraging pre-trained image captioning models, the ``Image Captioner'' module produces captions for the input image.

\textbf{Text Detector} ($M_{td}$): This module is designed to identify text within a given image. Typically, the ``Text Detector'' is employed when a question requires the extraction of textual information from images containing diagrams, charts, tables, maps, or other visual elements. By effectively detecting text in various formats, this module aids in the analysis and understanding of image-based content.
% and the "has image" field in the metadata is True.


\textbf{Row Lookup} ($M_{rl}$): In situations where questions involve tabular context, locating relevant cells to answer the question is often necessary. Large tables with numerous cells can potentially distract the system when attempting to comprehend the data. The ``Row Lookup'' module addresses this challenge by returning a simplified version of the table, retaining only the rows pertinent to the question. This module accepts a question and a table as input and outputs the simplified table. If all rows are relevant, the original table is returned.

\textbf{Column Lookup} ($M_{cl}$): Similar to the ``Row Lookup'' module, the ``Column Lookup'' module is designed to handle questions involving tabular context by focusing on relevant columns. This module streamlines the table by retaining only the columns that are pertinent to the question. The table keeps the same if all columns are relevant.

\textbf{Table Verbalizer} ($M_{tv}$): Since the LLM is fundamental to our system, converting structured tables into text is likely to enhance the comprehension of tabular information by various downstream modules as shown by \cite{ma-etal-2022-open} for open-domain question answering. Thus, the module is introduced to convert tables into easily comprehensible descriptions for downstream modules like ``Program Generator'' and ``Solution Generator''. This module is typically employed when the table has a small number of rows and columns and is domain-specific, such as stem-and-leaf plots or function tables. By transforming tabular data into natural language, this module facilitates better understanding and processing by subsequent modules.

\textbf{Program Generator} ($M_{pg}$): Recent work has shown that program-aided approaches are able to improve the logical and mathematical reasoning abilities of large language models \cite{wang2022code4struct,gao2022pal,chen2022program,mishra2022lila,imani2023mathprompter,paranjape2023art}.
Taking the question and context, the ``Program Generator'' module generates Python programs that can solve the given question effectively. This module is particularly useful when questions and contexts involve complex computations, such as arithmetic operations on multiple numbers, or when questions require intricate logical operations, such as ``if-else'' statements.


\textbf{Program Verifier} ($M_{pv}$): Recent work emphasizes the contribution of the verifying generation to reduce hallucination \cite{peng2023check,madaan2023self}. Therefore, the ``Program Verifier'' is designed to ensure the validity and error-free nature of the programs generated by the ``Program Generator''. The ``Program Verifier'' checks for syntax errors, logical errors, and other potential issues that may arise during program execution, improving the overall reliability and accuracy of the generated solutions.

\textbf{Program Executor} ($M_{pe}$): This module executes the program generated by ``Program Generator'' and produces the result, bridging the gap between program generation and final solution derivation. 

% \textbf{Solution Generator} ($M_{sg}$): The ``Solution Generator'' module is designed to generate a detailed solution to the input question, considering all the information stored in the cache. This module produces solutions in a chain-of-thought prompting manner, as proposed by \cite{wei2022chain}, ensuring a coherent and well-structured response based on the available information. The planner can rely on this module only if the  planner has high confidence to solve it by itself.

\textbf{Solution Generator} ($M_{sg}$): The ``Solution Generator'' module aims to generate a detailed solution to the input query, taking into account all the information stored in the cache. Employing a chain-of-thought prompting approach \cite{wei2022chain}, this module ensures coherent and well-structured responses based on the available information. The planner relies on this module only if this module is powerful enough to solve the problem independently, especially for simple problems.

\textbf{Answer Generator} ($M_{ag}$): This task-specific module extracts and normalizes the answer from the results generated by the ``Program Executor'' or ``Solution Generator'' using a rule-based approach. Typically, the ``Answer Generator'' module serves as the final module in the reasoning pipeline of our~\model, ensuring a concise and appropriate response based on the preceding steps.


\subsection{Science Question Answering}
\label{sec:sqa}

Science Question Answering (\scienceqa \cite{lu2022learn}) is a multi-modal question-answering benchmark covering a wide range of scientific topics over diverse contexts. As illustrated in \autoref{fig:showcase_scienceqa}, answering questions in \scienceqa requires using various knowledge, tools, and skills, such as image captioning, text detection, external knowledge retrieval, online resource search, and visual reasoning based on multiple clues. When generating programs for using tools, we constrain the search space to the relevant part of the entire inventory, as listed in \autoref{tab:tools_task}. 

Programs are deemed invalid if the modules ``Solution Generator'' and ``Answer Generator'' are not the final two elements. Invalid programs are then set to the default program, consisting of a sequence of ``Solution Generator'' and ``Answer Generator'', which refers to the chain-of-thought prompting baseline \cite{wei2022chain}. The constructed prompt for the natural language planner is displayed in \autoref{fig:policy_scienceqa}. The prompts for LLM-based modules, such as ``Knowledge Retrieval'', ``Query Generator'', and ``Solution Generator'' are  shown in \autoref{fig:policy_scienceqa_kr},  \autoref{fig:policy_scienceqa_qg}, and \autoref{fig:policy_scienceqa_sg}, respectively.

\subsection{Tabular Mathematical Reasoning}
\label{sec:tabmwp}

\tabmwp \cite{lu2023dynamic} is a mathematical reasoning task on tables. There are diverse tabular contexts, including schedules, prices, tax forms, plots, and function relations. As the examples shown in \autoref{fig:showcase_tabmwp}, this task requires AI systems to understand tables of various forms from different domains and perform precise numerical/symbolic computations. Similar to \scienceqa, we again constrain the program search space to focus on two types of tools, particularly, 1) tools can help LLMs better digest tabular information, e.g., ``Row Lookup'', ``Column Lookup'',  and ``Table Verbalizer''; 2) tools can perform faithful symbolic computations, such as ``Program Generator'', ``Program Verifier'', and ``Program Executor''. %, as well as ``Knowledge Retrieval'' to obtain domain-specific knowledge.
The full list is shown on the right side of \autoref{tab:tools_task}.

The generated programs adhere to additional constraints, such as the inclusion of ``Answer Generator'', the placement of ``Program Generator'' prior to ``Program Verifier'', and the positioning of ``Program Generator'' before ``Program Executor''. If these conditions are not met, the programs are regarded as invalid and set as a sequence of ``Program Generator'', ``Program Verifier'', ``Program Executor'', and ``Answer Generator''. This program corresponds to the program-of-thought prompting baseline \cite{chen2022program} with added program verification.


%\newpage
\section{Experiments}
\label{sec:experiment}

We conduct experiments on two complex reasoning tasks, \scienceqa \cite{lu2022learn} and \tabmwp \cite{lu2023dynamic}, to evaluate our \model in terms of effectiveness and adaptability.

\begin{table*}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/tools_task.pdf}
    \caption{Tools used on \scienceqa and \tabmwp, respectively. The reusable tools in two tasks are highlighted in \textcolor{Green}{\textbf{green}}.}
    \label{tab:tools_task}
    % \vspace{-10mm}
\end{table*}

\subsection{Experimental Setup}

\textbf{Planner implementations.} We choose the \textit{gpt-3.5-turbo} engine for ChatGPT and the \textit{gpt-4} engine for GPT-4 when constructing the LLM-based planner. The maximum length for generated programs is set to 128, and the temperature is set to 0 for the most deterministic generation.



\textbf{Modules implementations.}  
The ``Bing Search'' module calls the Bing Search API\footnote{\text{\url{https://www.microsoft.com/bing}}} and returns the top three responses for the text query. For the ``Image Captioner'' module, we use the captioning model \footnote{\text{\url{https://huggingface.co/nlpconnect/vit-gpt2-image-captioning}}} to generate textual descriptions for input images. The maximum length of generated captions is set to 16, the number of beams is 4, and the maximum number of output tokens is 512. The ``Text Detector'' tool is based on the github model
\footnote{\text{\url{https://github.com/JaidedAI/EasyOCR}}} to extract the text contents with coordinates in the image.
The ``Row Lookup'' module is enabled only when there are more than three rows and 18 table cells, in order to accelerate inference. Similarly, the Column Lookup'' module is enabled with two or more columns and 18 or more table cells. On \scienceqa, the Answer Generator'' module extracts the answer snippet from the result provided by the Solution Generator'' and selects the most similar option from the given choices. For \tabmwp, the ``Answer Generator'' is used to normalize answers with two-place precision for questions with numerical answers and select the most similar option for multiple-choice questions. For more details, please refer to our code implementations at \textbf{\url{https://github.com/lupantech/chameleon-llm}}.

\subsection{Experimental Results}

% Table
\input{tables/results_scienceqa}

\begin{figure*}[t!] 
  \begin{minipage}{0.50\textwidth} 
    \centering
    \includegraphics[width=1.0\textwidth]{figs/scienceqa_bar.pdf}
    \caption*{(a) Results on \scienceqa} 
  \end{minipage}
  \hfill
  \begin{minipage}{0.50\textwidth} 
    \centering
    \includegraphics[width=1.0\textwidth]{figs/tabmwp_bar.pdf}
    \caption*{(b) Results on \tabmwp} 
  \end{minipage}
  \caption{Performance comparison of main baselines and our \model on \scienceqa and \tabmwp. The vertical dashed line represents human performance and * represents models fine-tuned in multi-modal settings. On \scienceqa, \model using GPT-4 surpasses the previously published best few-shot model and attains results comparable to fine-tuned models. On \tabmwp, \model with GPT-4 achieves state-of-the-art results, exceeding human performance by 8.6\%.}
  \label{fig:results_highlight}
\end{figure*}


\textbf{\scienceqa.} \autoref{tab:scienceqa} presents the results of existing baselines and our \model, with key findings highlighted in \autoref{fig:results_highlight} (a). Employing ChatGPT \cite{openai2022chatgpt} as the base LLM, our \model achieves an overall accuracy of 79.93\%, a 1.62\% improvement over Chain-of-Thought (CoT) \cite{wei2022chain} prompted ChatGPT. Notably, \model is a generalized form of CoT, where the generated program is a sequence of ``Solution Generator'' and ``Answer Generator''. \model benefits from additional tool usage, such as ``Knowledge Retrieval'', ``Bing Search'', ``Image Captioner'', and ``Text Detector''. When built upon GPT-4 \cite{OpenAI2023GPT4TR}, our model attains an accuracy of 86.54\%, outperforming GPT-4 CoT \cite{lu2022learn} by 2.55\% and GPT-3 CoT by 11.37\%, creating the new state of the art in the few-shot setting.


% \pan{Analyze the accuracy scores with different settings: enabled/disabled some modules, accuracy among different groups of a number of table cells, accuracy for questions with/without the text in the image, and so on.}


% Table
\input{tables/results_tabmwp}

% \pan{Specialize the selection and implementation of modules }

\textbf{\tabmwp.} Results are shown in \autoref{tab:tabmwp}, with key models highlighted in \autoref{fig:results_highlight} (b). Similar significant improvements are observed for \model over both fine-tuned and few-shot prompted models. It is worth noting that both CoT and Program-of-Thought (PoT) \cite{chen2022program} can be viewed as special cases of \model. Specifically, CoT does not use any tool whereas PoT only resorts to symbolic programming tools in our inventory, e.g., ``Program Generator'', ``Program Executor'', and ``Answer Generator''. \model (ChatGPT) achieves improvements of 11.25\% and 3.79\% over ChatGPT CoT and ChatGPT PoT, respectively, demonstrating the advantage of our enriched tool set. By updating the underlying LLM with GPT-4, our \model achieves a further gain of 5.50\%, resulting in a 98.78\% accuracy. Remarkably, our \model (GPT-4) not only surpasses the previous best-performing model (Codex PoT-SC \cite{chen2022program}) by 17.0\%, but also outperforms the human performance by 8.56\%.


\subsection{Qualitative Analysis}

\begin{table*}[t!] 
 \centering
 % \normalsize
 \small
 % \renewcommand\tabcolsep{4.0pt} % column space
 % \renewcommand\arraystretch{1.1} % row space
 % \resizebox{1.0\linewidth}{!}{
 \begin{tabular}{llcc} 
 \toprule
 \header{Task} & \header{Model} & \header{\# of different programs} & \header{Average program length} \\
 \midrule
 \multirow{3}{*}{\scienceqa} & Chain-of-thought (CoT)  & 1 & 2 \\
 & \modelchatgpt & 14 & 3.03 \\
 & \modelgpt & 11 & 3.40 \\
 \midrule 
 \multirow{4}{*}{\tabmwp} & Chain-of-thought (CoT) & 1 & 2 \\
 & Program-of-thought (PoT) & 1 & 3 \\
 & \modelchatgpt & 28 & 4.17 \\
 &\modelgpt  & 19 & 4.09 \\
 \bottomrule
 \end{tabular}
 % }
 \caption{The statistics of the number of different generated programs and the average length of generated programs by our \model, respectively. Chain-of-thought (CoT) prompting and Program-of-thought (PoT) prompting are also compared as they are the special cases of \model.}
 \label{tab:tool_num}
\end{table*}

\noindent\textbf{Generated program statistics.} \model utilizes the LLM-based natural language planner to generate programs, i.e., sequences of used modules (tools). We report the statistics of the number of unique generated programs and the average length of corresponding tool sequences by our \model in \autoref{tab:tool_num}. On both \scienceqa and \tabmwp, using GPT-4 as the base LLM generates fewer distinct programs, i.e., more consistent programs, than using ChatGPT, even when given the exact same prompt in the planning model. Our results are consistent with the findings in \cite{OpenAI2023GPT4TR}, which observes that GPT-4 has a superior capability of understanding long contexts, aligning with human instructions, and performing high-level reasoning compared to other LLMs such as ChatGPT.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/tool_call_scienceqa.pdf}
    \caption{Tools called in the generated programs from \model (ChatGPT) and \model (GPT-4) on \scienceqa.}
    \label{fig:tool_call_scienceqa}
\end{figure*}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/tool_call_tabmwp.pdf}
    \caption{Tools called in the generated programs from \model (ChatGPT) and \model (GPT-4) on \tabmwp.}
    \label{fig:tool_call_tabmwp}
\end{figure*}

\noindent\textbf{Tool use planning.} We visualize the proportions of key tools called and not called in the generated programs from \model (ChatGPT) and \model (GPT-4) on \scienceqa (shown in \autoref{fig:tool_call_scienceqa}) and on \tabmwp (shown in \autoref{fig:tool_call_tabmwp}, respectively. Interestingly, ChatGPT and GPT-4 exhibit different planning behaviors. Generally, ChatGPT has a strong bias toward using or not using certain tools, which is highly influenced by the bias from in-context examples. For instance, ChatGPT calls ``Knowledge Retrieval'' in 72\% of queries but only calls ``Bing Search'' in 3\% of cases on \scienceqa; similarly, ChatGPT heavily relies on ``Row Lookup'' (59\%) but calls ``Column Lookup'' less frequently (5\%). However, GPT-4 acts more \textit{objectively} and \textit{rationally} when determining which tool to use or not. For example, GPT-4 calls ``Knowledge Retrieval'' more frequently (81\% vs. 72\%) and calls ``Bing Search'' more than ChatGPT (11\% vs. 3\%) when answering scientific questions on \scienceqa. More impressively, GPT-4 consistently calls ``Query Generator'' and ``Bing Search'' simultaneously by observing the language descriptions of tool use, while ChatGPT lacks such reasoning capability.


%\pan{Transitions}

We visualize the transition graphs of modules for generated programs by \model (GPT-4) on \scienceqa and \tabmwp in \autoref{tab:transition_scienceqa} and \autoref{tab:transition_tabmwp} respectively.
The transition probabilities in these graphs are computed from the tool transitions observed on the test sets of these two datasets. These graphs illustrate that the GPT-4 planner is able to make good decisions on how to sequence tools in a few-shot setup. For example on ScienceQA, \model often decides to rely on either the knowledge retriever or Bing search, but rarely both. On TabMWP, we observe two main modes: either going through the solution-executor module, or via the program verifier and executor.  


% \include{tables/tool_num}

\subsection{Case Study} 

Three examples from \model (GPT-4) on \scienceqa are visualized in \autoref{fig:showcase_scienceqa}. \model (GPT-4) is able to adapt to different input queries by generating programs that compose various tools and executing them sequentially to obtain the correct answers. For instance, to answer the first question, ``\textit{What is the direction of this push?}'', the system calls the image captioner model to extract semantic information from the image and employs the knowledge retrieval model to gather background knowledge for multi-modal reasoning. In the second example, the natural language planner infers that a text detector tool is needed to understand the context of the ad. In the third example (with more details provided in \autoref{fig:showcase_scienceqa_more} in the appendix), the query asks, ``\textit{Which animal's skin is adapted for survival in cold places?}'', which involves scientific terminology related to animal survival. Consequently, the planner decides to rely on the Bing search engine for domain-specific knowledge, benefiting from the numerous online resources available.

The adaptability and versatility of our \model for various queries are also observed on \tabmwp, as illustrated in the examples in \autoref{fig:showcase_tabmwp}. The first example involves mathematical reasoning on a tax form. \model (1) calls the knowledge retrieval model to recall basic knowledge that assists in understanding such domain-specific tables, (2) describes the table in a more readable natural language format, and (3) finally relies on program-aided tools to perform precise computations. In the second example, the system generates Python code that closely aligns with the background knowledge provided by the knowledge retrieval model. The third example requires the system to locate the cell in a large tabular context given the input query. \model calls the row lookup model to help accurately locate the relevant rows and generate the language solution via an LLM model, instead of relying on program-based tools.


% \pan{Failure Cases}

% \pan{Analyze the accuracy scores with different settings: enabled/disabled some modules, accuracy among different groups of a number of table cells, accuracy for questions with/without the text in the image, and so on.}

% \subsection{Case Study: XXX}

% \pan{Add one demo from the team.}

% \subsection{Case Study: XXX}

% \pan{Add one more demo from the team.}

%\newpage
% \section{Future Work}
% \label{sec:future}


%\newpage
\section{Conclusion}
\label{sec:conclusion}

In conclusion, we have introduced a novel \textit{plug-and-play compositional} reasoning framework, \model, that leverages large language models to overcome the inherent limitations of current tool-augmented LLMs. Our approach employs a diverse set of tools and demonstrates impressive adaptability and effectiveness on two challenging benchmarks, \scienceqa and \tabmwp. By achieving significant improvements in accuracy over existing few-shot and state-of-the-art models, \model showcases its potential for addressing real-world queries across various domains. As research continues to advance in large language models and tool integration, we anticipate that our framework will serve as a foundation for further innovations in pursuing more generalizable and efficient solutions to complex reasoning tasks.

% \pan{future work, discuss the self-programming idea?} 




%%%%%%%%% Acknowledgment
% \clearpage
\section{Acknowledgment}
We would like to thank Chunyuan Li, Qiuyuan Huang, and other members of the Deep Learning group at Microsoft Research for their valuable discussions.


%%%%%%%%% REFERENCES
% \clearpage
\bibliographystyle{plain} 
{
\small
\bibliography{egbib}
% \nocite{*}
}



==> v2_arxiv_backup/app.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hrule height 4pt
\vskip 0.25in
\vskip -\parskip
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \fontsize{24pt}{\baselineskip}\selectfont {
% Supplementary Materials for \\ \hspace*{\fill} \\ IconQA: A New Benchmark for Abstract Diagram Understanding and Visual Language Reasoning}
\vbox{
    \centering
    \LARGE 
    \textbf{Supplementary Materials for \\  
    \model: Plug-and-Play Compositional Reasoning with Large Language Models}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vskip 0.29in
\vskip -\parskip
\hrule height 1pt
% \vskip 0.09in
% \vskip 0.15in
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand*\footnoterule{} % remove the separator line

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

% \blfootnote{
%     \footnotesize 
%     % \\37th Conference on Neural Information Processing Systems (NeurIPS 2023).
%     \\Submitted to 37th Conference on Neural Information Processing Systems (NeurIPS 2023). Do not distribute.

% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Appendix}
\label{app}

% This appendix includes
% \begin{itemize}
%     \item Implementation details including the planner policy and module configurations (Sec. \ref{app:exp_details})
%     \item More qualitative results on \scienceqa (Sec. \ref{app:case_study_scienceqa})
%     \item More qualitative results on \tabmwp (Sec. \ref{app:case_study_tabmwp})
%     % more  qualitative  results
% \end{itemize}



\subsection{Current Tool-Augmented LLMs}
\label{app:tool_augmented}
To address the limitations of LLMs, an active research direction involves augmenting language models with access to external tools and resources, as well as exploring the integration of external tools and plug-and-play modular approaches. For example, aided by web search engines and  external knowledge resources, LLMs are able to access real-time information and leverage
domain-specific knowledge \cite{nakano2021webgpt}. To enhance mathematical reasoning abilities, recent work uses LLMs \cite{chen2021evaluating} to generate complex programs to exploit powerful computational resources, and execute logical reasoning tasks more effectively \cite{wang2022code4struct,gao2022pal,chen2022program,mishra2022lila,imani2023mathprompter,paranjape2023art}. Another line of recent work, such as ViperGPT \cite{suris2023vipergpt}, Visual ChatGPT \cite{wu2023visual}, VisProg \cite{gupta2022visual}, and HuggingGPT \cite{shen2023hugginggpt} incorporates a collection of foundation computer vision models to equip LLMs with the abilities to perform visual reasoning tasks.


\subsection{Experimental Details}
\label{app:details}

\paragraph{Module search space.} The inventory subsets for \scienceqa and \tabmwp are shown in Table \ref{tab:tools_task}.

\begin{table*}[!ht]
    \centering
    \includegraphics[width=0.99\linewidth]{figs/tools_task.pdf}
    \caption{Tools used on \scienceqa and \tabmwp, respectively. Reusable tools are marked in \textcolor{Green}{\textbf{green}}.}
    \label{tab:tools_task}
    % \vspace{-10mm}
\end{table*}

\paragraph{Planner implementations.} We choose the \textit{gpt-3.5-turbo} engine for ChatGPT and the \textit{gpt-4} engine for GPT-4 when constructing the LLM-based planner. The maximum length for generated programs is set to 128, and the temperature is set to 0 for the most deterministic generation. The planner prompts for the \scienceqa and \tabmwp are illustrated in Table \ref{fig:planner_scienceqa} and Table \ref{fig:planner_tabmwp}, respectively.

% \input{tables/planner_scienceqa}

% \input{tables/planner_tabmwp}

\paragraph{Module implementations for ScienceQA.} By default, the LLM-based models use four in-context examples as demonstrations, have a temperature setting of 0, and allow a maximum of 512 tokens for completion. Additional specific implementation details are provided as follows:

\begin{itemize}
    \item \textbf{Knowledge Retrieval}: The prompt consists of 3 demonstration examples and the template is shown in Table \ref{fig:planner_scienceqa_kr}. 
    \item \textbf{Query Generator}: The prompt template is shown in Table \ref{fig:planner_scienceqa_qg}. The maximum number of tokens for completion is set as 64. 
    \item \textbf{Solution Generator}: The prompt consists of 2 demonstration examples and the template is shown in Table \ref{fig:planner_scienceqa_sg}.
    \item \textbf{Image Captioner}: We use the captioning model\footnote{\text{\url{https://huggingface.co/nlpconnect/vit-gpt2-image-captioning}}} to generate textual descriptions for input images. The maximum length of generated captions is set to 16, the number of beams is 4, and the maximum number of output tokens is 512. 
    \item \textbf{Text Detector}: This module is based on the github model\footnote{\text{\url{https://github.com/JaidedAI/EasyOCR}}} to extract the text contents with coordinates in the image.
    \item \textbf{Bing Search}: This module calls the Bing Search API\footnote{\text{\url{https://www.microsoft.com/bing}}} and returns the top three responses for the text query. 
    \item \textbf{Answer Generator}: This module extracts the answer snippet from the result provided by the ``Solution Generator'' and selects the most similar option from the given choices. 
\end{itemize}


\paragraph{Module implementations for TabMWP.} Similar to \scienceqa, the LLM-based modules by default use four in-context examples as demonstrations, have a temperature setting of 0, and allow a maximum of 512 tokens for completion. Additional implementation details are provided as follows:
\begin{itemize}
    \item \textbf{Knowledge Retrieval}: The prompt consists of 5 demonstration examples and the template is shown in Table \ref{fig:planner_tabmwp_kr}.
    \item \textbf{Row Lookup}: This module is enabled only when there are more than three rows and 18 table cells, in order to accelerate inference. The prompt consists of 7 demonstration examples and the template is shown in Table \ref{fig:planner_tabmwp_rl}. The maximum number of tokens for completion is set as 256.
    \item \textbf{Column Lookup}: Similarly, this module is enabled with two or more columns and 18 or more table cells.  The prompt consists of 6 demonstration examples and the template is shown in Table \ref{fig:planner_tabmwp_cl}. The maximum number of tokens for completion is set as 256.
    \item \textbf{Table Verbalizer}: The prompt consists of 7 demonstration examples and the template is shown in Table \ref{fig:planner_tabmwp_tv}. 
    \item \textbf{Program Generator}: The prompt template is shown in Table \ref{fig:planner_tabmwp_pg}. The maximum number of tokens for completion is set as 256.
    \item \textbf{Solution Generator}:  The prompt consists of 16 demonstration examples and the template is shown in Table \ref{fig:planner_tabmwp_sg}. 
    \item \textbf{Answer Generator}: This module is used to normalize answers with two-place precision for questions with numerical answers and select the most similar option for multiple-choice questions.
\end{itemize}

% For more details, please refer to our code implementations at \textbf{\url{https://github.com/lupantech/chameleon-llm}}.

\subsection{Experimental Results}
\label{app:results}

\paragraph{Generated program statistics.} \model utilizes the LLM-based natural language planner to generate programs, i.e., sequences of used modules (tools). We report the statistics of the number of unique generated programs and the average length of corresponding tool sequences by our \model in Table \ref{tab:tool_num}. On both \scienceqa and \tabmwp, using GPT-4 as the base LLM generates fewer distinct programs, i.e., more consistent programs, than using ChatGPT, even when given the exact same prompt in the planning model. Our results are consistent with the findings in \cite{OpenAI2023GPT4TR}, which observes that GPT-4 has a superior capability of understanding long contexts, aligning with human instructions, and performing high-level reasoning compared to other LLMs such as ChatGPT.

\begin{table*}[ht!] 
 \centering
 % \normalsize
 \small
 % \renewcommand\tabcolsep{4.0pt} % column space
 % \renewcommand\arraystretch{1.1} % row space
 % \resizebox{1.0\linewidth}{!}{
 \begin{tabular}{llcc} 
 \toprule
 \header{Task} & \header{Model} & \header{\# of different programs} & \header{Average program length} \\
 \midrule
 \multirow{3}{*}{\scienceqa} & Chain-of-thought (CoT)  & 1 & 2 \\
 & \modelchatgpt & 14 & 3.03 \\
 & \modelgpt & 11 & 3.40 \\
 \midrule 
 \multirow{4}{*}{\tabmwp} & Chain-of-thought (CoT) & 1 & 2 \\
 & Program-of-thought (PoT) & 1 & 3 \\
 & \modelchatgpt & 28 & 4.17 \\
 &\modelgpt  & 19 & 4.09 \\
 \bottomrule
 \end{tabular}
 % }
 \caption{The statistics of the number of different generated programs and the average length of generated programs by our \model, respectively. Chain-of-thought (CoT) prompting and Program-of-thought (PoT) prompting are also compared as they are the special cases of \model.}
 \label{tab:tool_num}
\end{table*}


\paragraph{Visualization examples of \tabmwp.} 
The adaptability and versatility of our \model for various queries are also observed on \tabmwp, as illustrated in the examples in Figure \ref{fig:showcase_tabmwp}. The first example involves mathematical reasoning on a tax form. \model (1) calls the knowledge retrieval model to recall basic knowledge that assists in understanding such domain-specific tables, (2) describes the table in a more readable natural language format, and (3) finally relies on program-aided tools to perform precise computations. In the second example, the system generates Python code that closely aligns with the background knowledge provided by the knowledge retrieval model. The third example requires the system to locate the cell in a large tabular context given the input query. \model calls the row lookup model to help accurately locate the relevant rows and generate the language solution via an LLM model, instead of relying on program-based tools.


\section{Limitations} 
\label{app:limitations}
While \model represents a significant stride in exploiting large language models (LLMs) for compositional reasoning in a plug-and-play manner, there are a few areas that could benefit from further refinement. One such area is the expansion of its adaptability to a wider variety of tasks and domains, beyond the benchmarks presented. The LLM-based planner, responsible for synthesizing programs and determining the sequence of tools, introduces an innovative approach, yet it also raises intriguing research questions about optimizing the process for tool selection and sequence. It is plausible in the current system design that the quality of the LLM-based planner could impact overall performance. Moreover, \model generates the program at one step, without incorporating a re-planning mechanism as the modules in the program are processed. Furthermore, we make the assumption that the list of modules and their descriptions will fit within the context window of LLMs, which may not always be the case. As the task complexity increases and the module inventory expands, there might be a corresponding surge in computational demands or limitations due to the context limit, indicating potential areas for future optimization. However,  these potential areas for enhancement don't detract from the paper's central achievements, but instead provide valuable directions for future work and research.

% Firstly, the adaptability of Chameleon to new, unseen domains or tools is yet to be fully explored. While the paper demonstrates impressive performance on the chosen benchmarks, 
% its generalization ability across a broader range of tasks and domains is unclear. Secondly, the system's reliance on LLMs to synthesize programs raises concerns about the potential for introducing biases present in the training data of these LLMs. Thirdly, the selection and ordering of tools in the proposed approach is handled by the LLM-based planner, raising questions about the optimality of the sequence. The system's performance may be constrained by the quality of the LLM-based planner, making it sensitive to the specific LLM used. Lastly, the system's complexity might result in higher computational costs, which can be prohibitive for practical applications. Future work could address these limitations by conducting more extensive tests across diverse tasks and domains, examining ways to mitigate biases, improving the tool selection process, and optimizing the system for computational efficiency.
% \pan{Wu: Is it possible to re-plan as we go through the modules?}


\section{Broader Impacts}
\label{app:impacts}
The work presented in this paper, \model, has significant potential for positive societal impact. By augmenting large language models (LLMs) with plug-and-play modules for compositional reasoning, \model can provide more accurate responses to complex, multi-modal tasks, making it a potentially valuable framework for various applications, including but not limited to education, finance, and decision support systems. Additionally, the system's ability to synthesize programs without requiring any training could democratize access to AI technology, enabling non-experts to leverage the power of AI in diverse fields. As research continues to advance in large language models and tool integration, we anticipate that our framework will serve as a foundation for further innovations in pursuing more generalizable and efficient solutions to complex reasoning tasks.  

While there might be negative societal impacts associated with the \model, such as misinformation and privacy concerns if data sources and external tools it utilizes are not curated meticulously, we believe these risks can be carefully managed and minimized. There's also a risk that excessive reliance on \model's increased autonomy may undermine critical thinking skills or job functions. To effectively mitigate these issues, careful curation of data sources and external tools, along with a strong commitment to user data protection, are essential. Additionally, \model's autonomy should be viewed as a means to augment, not replace, human capabilities. Therefore, the development of robust ethical guidelines, transparency mechanisms, and safeguards is critical, underlying our commitment to the socially responsible deployment of AI.

% While we must be aware of potential negative societal impacts, we believe that these can be addressed effectively. For instance, the improved reasoning capabilities of \model could enhance the quality and reliability of information dissemination, provided that the data sources and external tools it leverages are curated carefully. The increased autonomy offered by \model should be seen as an opportunity to augment human capabilities, complementing rather than replacing critical thinking skills or job functions. In the context of privacy, \model's use of web search engines and other external tools is conducted with a strong commitment to respect user data and privacy. Consequently, this necessitates the ongoing development of robust ethical guidelines, transparency mechanisms, and safeguards, underlining our commitment to socially responsible AI deployment.

% responsible and ethical AI deployment.
% \model's improved reasoning capabilities could inadvertently be used to spread misinformation if the underlying data or external tools it draws upon are inaccurate or biased. Furthermore, as the system becomes more autonomous and capable, there's a risk of over-reliance on the technology, potentially leading to a reduction in critical thinking skills or job displacement in certain sectors. In terms of privacy, the use of web search engines and other external tools could also potentially expose sensitive information. It is therefore essential to have robust ethical guidelines, transparency mechanisms, and safeguards in place to prevent misuse and protect users' privacy.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/tool_call_bar_tabmwp.pdf}
    \caption{Tools called in the generated programs from \model (ChatGPT) and \model (GPT-4) on \tabmwp.}
    \label{fig:tool_call_tabmwp}
\end{figure*}


\input{tables/planner_scienceqa}

\input{tables/planner_tabmwp}

\input{tables/planner_tools}

\begin{figure*}[th!]
    \centering
    \includegraphics[width=0.65\linewidth]{figs/sqa-gpt4.pdf}
    \caption{Transitions between modules in programs generated by \model (GPT-4) on \scienceqa.  START is the start symbol, END is a terminal symbol and the others are non-terminal symbols.}
    \label{fig:transition_scienceqa}
\end{figure*}

\begin{figure*}[th!]
    \centering
    \includegraphics[width=0.80\linewidth]{figs/tabmwp-gpt4.pdf}
    \caption{Transitions between modules in programs generated by \model (GPT-4) on \tabmwp. START is the start symbol, END is a terminal symbol and the others are non-terminal symbols.}
    \label{fig:transition_tabmwp}
\end{figure*}

\begin{figure*}[th!]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/showcase_scienceqa_more.pdf}
    \caption{One more example from our \model (GPT-4) on \scienceqa.}
    \label{fig:showcase_scienceqa_more}
\end{figure*}

\begin{figure*}[th!]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/showcase_tabmwp_one.pdf}
    \caption{One more example from our \model (GPT-4) on \tabmwp.}
    \label{fig:showcase_tabmwp_one}
\end{figure*}


\input{tables/failure}




\clearpage
\subsection{Error Analysis}

To examine the error sources of the base large language models and understand how our model reduces mistakes from different aspects, we conduct an error analysis, as shown in Figure \ref{fig:error_analysis_scienceqa}. We select 50 mistake examples from the ChatGPT baseline on \textsc{ScienceQA} as the evaluation set. We count the number of mistake examples and analyze their corresponding mistake type categories for ChatGPT, our \model (ChatGPT), and our \model (GPT-4). 

The results show that our \model approach can substantially reduce the number of mistakes compared to ChatGPT. Our model features tools for image captioning and knowledge retrieval, thus the mistakes made by ChatGPT in the category of image understanding are reduced to 10 and 19 from 32 by \model (ChatGPT) and  \model (GPT-4); while the mistakes made by ChatGPT in the category of knowledge understanding are reduced to 6 and 3 from 37 by \model (ChatGPT) and \model (GPT-4). Benefiting from the sequential execution of tools, the mistakes caused by solution generation are significantly reduced as well. Additionally, we find that the task planning of GPT-4 outperforms ChatGPT by a large margin.

\begin{figure*}[th!]
    \centering
    \includegraphics[width=0.85\linewidth]{figs/error_analysis_scienceqa.pdf}
    \caption{Number of mistake examples in different categories from ChatGPT, our \model (ChatGPT), and  \model (GPT-4) on \scienceqa. Image: image captioning, Knowledge: knowledge understanding, Solution: solution generation.}
    \label{fig:error_analysis_scienceqa}
\end{figure*}




==> v2_arxiv_backup/body.tex <==
%%%%%%%%% BODY TEXT

\section{Introduction}
\label{sec:intro}


% \pan{Recent progress of large language models, especially in the field of reasoning}
Remarkable progress has been observed in recent large language models (LLMs) for various natural language processing tasks, with prominent examples such as GPT-3 \cite{brown2020language}, PaLM \cite{chowdhery2022palm}, LLaMA \cite{llamaadapter2023}, ChatGPT \cite{openai2022chatgpt}, and the recently developed GPT-4 \cite{OpenAI2023GPT4TR}. LLMs have demonstrated emergent abilities, including in-context learning and chain-of-thought (CoT) reasoning \cite{wei2022emergent}. These models are capable of solving diverse tasks in a zero-shot fashion \cite{kojima2022large} or with the aid of a few examples \cite{wei2022chain}, and they show great potential in planning and decision-making akin to human beings \cite{huanginner2022,huang2022language}. Despite these capabilities, LLMs face inherent limitations, such as an inability to access up-to-date information \cite{komeili2022internet}, perform precise mathematical reasoning \cite{patel2021nlp, lu2023dl4math}, or utilize specialized models \cite{schick2023toolformer}. 
Therefore, enhancing current LLMs with the capability to automatically \textit{compose} external tools for real-world task solving is critical to address these drawbacks.
% Thus, enhancing current LLMs with reasoning abilities from external tools has emerged as a new research topic \cite{qin2023tool}. However, the integration of different modules to perform complex tasks remains challenging and may require carefully curated rules, potentially leading to poor generalization in unseen situations.

% It is also challenging to integrate different modules to perform complex tasks, which might need carefully curated rules. 
% Additionally, integrating different modules to perform complex tasks can prove challenging and may require carefully curated rules for effective operation.
% Moreover, integrating different modules to accomplish complex tasks remains challenging, often necessitating carefully curated rules.

% \begin{figure}[th!]
%     \centering
%     \vspace{-4mm}
%     \includegraphics[width=0.99\linewidth]{figs/showcase_scienceqa.pdf}
%     \vspace{-1mm}
%     \caption{Examples from our~\model~with GPT-4 on \scienceqa \cite{lu2022learn}, a multi-modal question answering benchmark in scientific domains.~\model~is adaptive to different queries by synthesizing programs to compose various tools and executing them sequentially to get final answers.}
%     \label{fig:showcase_scienceqa}
%     \vspace{-4mm} 
% \end{figure}

% \pan{Recent attempts in tool use, analysis of the limitations of current work}
% To address these limitations of LLMs, an active research direction involves augmenting language models with access to external tools and resources, as well as exploring the integration of external tools and plug-and-play modular approaches. For example, aided by web search engines and  external knowledge resources, LLMs are able to access real-time information and leverage
% domain-specific knowledge \cite{nakano2021webgpt}. To enhance mathematical reasoning abilities, recent work uses LLMs \cite{chen2021evaluating} to generate complex programs to exploit powerful computational resources, and execute logical reasoning tasks more effectively \cite{wang2022code4struct,gao2022pal,chen2022program,mishra2022lila,imani2023mathprompter,paranjape2023art}. Another line of recent work, such as ViperGPT \cite{suris2023vipergpt}, Visual ChatGPT \cite{wu2023visual}, VisProg \cite{gupta2022visual}, and HuggingGPT \cite{shen2023hugginggpt} incorporates a collection of foundation computer vision models to equip LLMs with the abilities to perform visual reasoning tasks.

% Despite significant progress, current tool-augmented LLMs still face critical challenges when addressing real-world queries. Most existing approaches are either limited to a small number of tools \cite{mishra2022lila,chen2022program,wang2022code4struct,imani2023mathprompter,paranjape2023art,schick2023toolformer} or rely on domain-specific tools \cite{nakano2021webgpt,yang2023mm,gupta2022visual,wu2023visual,suris2023vipergpt}, and thus are not easy to generalize to diverse queries. 
Consider the example in Figure \ref{fig:showcase_scienceqa}: \textit{Which is the main persuasive appeal used in this ad?}. To answer this question, one needs to: 1) infer that there is an ad image containing text context and call a text decoder to understand the semantics; 2) retrieve background knowledge about \textit{persuasive appeals} and the differences among three persuasive appeals; 3) generate a solution based on the input query and intermediate results from previous steps; and 4) finally produce the answer in a task-specific format. On the other hand, when answering \textit{Which animal's skin is adapted for survival in cold places}, one might need to call modules such as an image captioner to decipher image information and a web search engine to retrieve domain knowledge to understand scientific terminologies. 
% To answer queries in Figure \ref{fig:showcase_tabmwp}, one needs to compose different tools to perform mathematical reasoning in a tabular context. 
However, current tool-augmented LLMs still face challenges when addressing these real-world queries across various scenarios. Most existing approaches are either limited to a small number of tools \cite{mishra2022lila,chen2022program,wang2022code4struct,imani2023mathprompter,paranjape2023art,schick2023toolformer} or relying on domain-specific tools \cite{nakano2021webgpt,yang2023mm,gupta2022visual,wu2023visual,suris2023vipergpt}, and thus are not easy to generalize to queries of new domains (see sections \ref{sec:related} and \ref{app:tool_augmented} for further discussion). In this work, we study how to enable LLMs to synthesize programs to capture the logic of composing heterogeneous tools.
% Earlier work does not systematically study how to compose heterogeneous tools with LLM, 

To address the challenges of existing work, we introduce~\model, a \textit{plug-and-play compositional} reasoning framework  that leverages LLMs to synthesize programs and compose various tools for a wide range of tasks.
Unlike existing tool-augmented LLMs \cite{schick2023toolformer, nakano2021webgpt,yang2023mm,gupta2022visual,wu2023visual,suris2023vipergpt}, \model uses a richer set of tools, including LLMs, off-the-shelf  vision models, web search engines, Python functions, and heuristics-based modules. Moreover, \model leverages the in-context learning capabilities of LLMs and builds on an LLM as a natural language planner, without requiring any training or carefully curated rules.
Prompted by tool descriptions and usage examples, the planner infers a program composed of a sequence of tools to execute in order to generate the final response for a user query. Instead of generating programs in domain-specific languages \cite{nakano2021webgpt, suris2023vipergpt, gupta2022visual}, \model generates natural-language-like (NL) programs (e.g., 
\texttt{[Text\_Detector, Knowledge\_Retrieval, Solution\_Generator, Answer\_Generator]} for the second query in Figure \ref{fig:showcase_scienceqa}). The NL-like programs are 
easy to understand and debug by users with limited programming experience, and easily extendable to new modules.
During each module's execution, the module processes the query and cached context, returns a result determined by the module itself, and updates the query and context for subsequent execution. Composing modules as a sequential program allows subsequent modules to leverage prior cached context and updated queries.
% tailored to specifically customized tasks
%less error-prone, easy to debug, user-friendly 

We showcase the adaptability and effectiveness of \model on two tasks: \scienceqa \cite{lu2022learn} and \tabmwp \cite{lu2023dynamic}. \scienceqa is a multi-modal question answering benchmark spanning multiple context formats and various scientific topics, while \tabmwp is a mathematical benchmark involving diverse tabular contexts. These two benchmarks serve as a good testbed to evaluate \model's ability to coordinate diverse tools across different types and domains. Notably, \model with GPT-4 achieves an 86.54\% accuracy on \scienceqa, significantly improving upon the best published few-shot model by 11.37\%. On \tabmwp, using GPT-4 as the underlying LLM, \model achieves an improvement of 7.97\% over chain-of-thought (CoT) prompted GPT-4 \cite{wei2022chain} and a 17.0\% increase over the best-published model \cite{chen2022program}, lifting the state of the art to 98.78\%. Further studies suggest that using GPT-4 as a planner exhibits more consistent and rational tool selection and is able to infer potential constraints given the instructions, compared to other LLMs like ChatGPT.

% \model built upon ChatGPT attains an accuracy of 93.28\%, an improvement of 11.25\% over the chain-of-thought (CoT) prompted ChatGPT. When 
% \pan{Differentiate our work?}

% (1) \textit{cross-task generalization}

% (2)\textit{ Easy to debug}

% (3) \textit{interpretable}

% (4) et al

% \red{We introduce V
% ISP
% ROG which inputs visual data (a sin- gle image or a set of images) along with a natural language instruction,  generates  a  sequence  of  steps,  a visual  pro- gram if you will, and then executes these steps to produce the desired output}

% \red{Modules may be off-the-shelf computer vi-
% sion  models,  language  models,  image  processing  subrou- tines  in  OpenCV  [4],  or  arithmetic  and  logical  operators.}

% Auto-GPT

% \pan{Summarize our contributions}
Our contributions are as follows:
(1) We develop a plug-and-play compositional reasoning framework, \model, that effectively composes external tools to address inherent limitations of LLMs and tackle a broad range of reasoning tasks. (2) Relying on an LLM as a natural language planner to generate programs, \model successfully integrates various tools, including LLMs, off-the-shelf vision models, web search engines, Python functions, and rule-based modules, to build a versatile and adaptable AI system capable of answering real-world queries. (3) We demonstrate \model's effectiveness on two challenging benchmarks, significantly surpassing the state of the art.
% \scienceqa and \tabmwp
% adaptability and 
%results. achieving significant improvement over the best published few-shot results.



\section{Related Work}
\label{sec:related}

\paragraph{Compositional Reasoning}

Neural modular and compositional approaches have been explored to automatically perform desired sub-task decomposition, enhancing interpretability and adaptability across various reasoning tasks. Early work \cite{andreas2016learning, andreas2016neural} posits that complex reasoning tasks are fundamentally compositional and proposes neural module networks (NMN) to decompose them into subtasks. However, these methods rely on brittle off-the-shelf parsers and are limited by module configurations. Some later work \cite{johnson2017inferring,hu2017learning,hu2018explainable,khot2021text}, takes a step further by predicting instance-specific network layouts in an end-to-end manner, without relying on parsers, using reinforcement learning \cite{williams1992simple} and weak supervised learning. % answer supervision. 
In visual reasoning, models comprising a program generator and an execution engine have been proposed to combine deep representation learning and symbolic program execution \cite{johnson2017inferring, yi2018neural}. In the domain of mathematical reasoning, an interpretable solver has been developed to incorporate theorem knowledge as conditional rules and perform symbolic reasoning step by step \cite{lu2021inter}.
Our work takes inspiration from neural module networks, yet it offers several distinct advantages. First,~\model~does not require expensive supervision of task-specific programs for modeling training. Instead, it generates sequential programs, consisting of modules, that are easy to generalize to various domains and tasks, allowing the extension to new modules in a plug-and-play manner. Second,~\model~does not require any training, but uses the in-context learning capabilities of LLMs to generate programs prompted by natural language instruction and demonstrations.


\begin{figure}[t!]
    \centering
    \vspace{-3mm}
    % \includegraphics[width=1.0\linewidth]{figs/showcase_tabmwp_long.pdf}
    \includegraphics[width=1.0\linewidth]{figs/showcase_tabmwp_two.pdf}    \caption{Two examples from our~\model~with GPT-4 on \tabmwp \cite{lu2023dynamic}, a mathematical reasoning benchmark with tabular contexts. \model demonstrates flexibility and efficiency in adapting to different queries that require various reasoning abilities.}
    \label{fig:showcase_tabmwp}
    \vspace{-3mm}
\end{figure}


\input{tables/comparison}

% \paragraph{Large Language Models}
% In recent years, the development of large language models (LLMs) has made tremendous progress, as evidenced by models such as BLOOM \cite{scao2022bloom}, PaLM \cite{chowdhery2022palm}, Flan-T5 \cite{chung2022scaling}, LLaMA \cite{touvron2023llama}, GPT-3 \cite{brown2020language}, ChatGPT \cite{openai2022chatgpt}, and GPT-4 \cite{OpenAI2023GPT4TR}. These LLMs exhibit emergent abilities, including in-context learning, mathematical reasoning, and commonsense reasoning. LLMs like GPT-3 and GPT-4 are capable of solving various tasks using zero or only a handful of task-relevant examples. The chain-of-thought (CoT) approach \cite{wei2022chain} instructs LLMs to decompose complex problems by generating intermediate reasoning steps before arriving at the final answer. Another active research area is to incorporate external verification \cite{peng2023check,madaan2023self} and human feedback \cite{openai2022chatgpt} to allow LLMs to perform more reliably and align better with human preferences. In addition, a recent line of work focuses on instruction learning, either via generating high-quality instructions data \cite{peng2023instruction} or by boosting the language models with instructions, such as Flan-T5 \cite{chung2022scaling}, LLaMA \cite{touvron2023llama}, LLaMA-Adapter \cite{llamaadapter2023}, and LLaVA \cite{liu2023llava}. Our proposed~\model~builds on these lines of work, introducing a general approach that enables cross-task generalization, leverages in-context learning from demonstrations, and integrates various capabilities of external tools to solve complex reasoning problems. 


\paragraph{Tool-Augmented Language Models}
In recent years, the development of large language models (LLMs) \cite{scao2022bloom,chowdhery2022palm,chung2022scaling,touvron2023llama,brown2020language,openai2022chatgpt,OpenAI2023GPT4TR} has made tremendous progress, and further stimulate the research in prompting learning \cite{wei2022chain,lu2023dynamic,khot2023decomposed} and instruction learning \cite{touvron2023llama,llamaadapter2023,peng2023instruction,gao2023llamaadapterv2}.
Despite the impressive performance of LLMs, %\cite{brown2020language,openai2022chatgpt} and demonstrate emergent capabilities \cite{wei2022emergent} across various natural language processing tasks. However, these language models also 
they suffer from inherent limitations, such as the inability to access up-to-date information \cite{komeili2022internet}, utilize external tools \cite{schick2023toolformer}, or perform precise mathematical reasoning \cite{patel2021nlp, lu2023dl4math}. To address these shortcomings, there has been a growing interest in exploring the use of external tools and modular approaches to augment LLMs. These augmented LLMs can access real-time information aided by web search engines \cite{nakano2021webgpt} and leverage domain-specific knowledge from external resources \cite{yu2023generate}.  Some work leverages the Python interpreter to generate complex programs to employ powerful computational resources, and execute logical reasoning tasks more effectively \cite{wang2022code4struct,gao2022pal,chen2022program,mishra2022lila,imani2023mathprompter,paranjape2023art,lu2023multimodal}.
For example, Toolformer \cite{schick2023toolformer} constructs tool-use augmented data to train language models to select five tools. In the realm of visual tools, various approaches have been proposed to enhance the capabilities of large language models in handling visual tasks \cite{yang2023mm,wu2023visual,suris2023vipergpt,gupta2022visual,shen2023hugginggpt}, augmented with Hugging Face models \cite{shen2023hugginggpt}, Azure models \cite{yang2023mm}, visual foundation models \cite{wu2023visual}.

We compare~\model~with other tool-augmented language models in Table \ref{tab:tool_comparison}. Many of these approaches are either constrained to a small set of tools or limited to task-specific tools, which reduces their capabilities across various skill dimensions and hampers their generalizability to new tasks. A recent line of work relies on large amounts of supervision \cite{schick2023toolformer, komeili2022internet} and focuses on generating commands \cite{nakano2021webgpt} and programs \cite{suris2023vipergpt,gupta2022visual} to infer the choice of tools. However, this approach needs to carefully tailor prompts to specific tasks and particular tools, and is neither flexible nor adaptive. 
%potentially hindering its flexibility and adaptability. 
In contrast,~\model~instructs LLMs with natural language instructions that simply describe the roles of each module and provide a few calling examples, eliminating the need for additional training or tool-specific prompts when learning to compose different tools. More importantly,~\model~offers users flexibility in terms of tool types and sources, updating the underlying LLMs, adding new tools, and adapting 
to new tasks. 
 % by updating the instructions
Our work shares the same spirit of AutoGPT \cite{autogpt2023}, an autonomous GPT-4 agent with the artificial general intelligence (AGI) ambition to incorporate numerous tools to achieve user-defined goals. While AutoGPT is still under development, our work is the first to instantiate the idea and verify its effectiveness on well-studied benchmarks.




\section{General Framework:~\model}

To address the limitations of current LLMs in utilizing diverse tools, we propose~\model~, a novel \textit{plug-and-play compositional} reasoning framework, synthesizing the composition of various tools to accommodate a wide range of problems. \model~is comprised of a module inventory that defines different types of tools and an LLM-based planner, whose purpose is to decompose the original problem into sub-tasks that can be effectively solved by task-specific tools.
Unlike existing tool-augmented LLM approaches~\cite{schick2023toolformer, gupta2022visual, wu2023visual,shen2023hugginggpt}, our module inventory features multiple tool types as illustrated in Table \ref{tab:tools}, enabling~\model~to exhibit various reasoning abilities, including image understanding, knowledge retrieval, web search, complex mathematical reasoning, and table understanding. 
Instead of generating domain-specific programs~\cite{nakano2021webgpt,gupta2022visual,suris2023vipergpt}, \model employs an LLM-based planner to create natural-language-like programs that follow natural language instructions, which is less error-prone, easily expandable to new modules, and user-friendly.

% Distinct from previous approaches, our~\model~method is capable of synthesizing the composition of various tools to accommodate a wide range of problems. It employs a natural language planner, $\cP$, to generate a sequential program to select and compose modules stored in an inventory, $\mathcal{M}$. Then, the program is executed to generate the answer. 

%the modules are bound and executed sequentially 
%\model~ enabling a flexible and adaptive problem-solving process.

% \subsection{Natural Language Planner}
% \pan{module definition, one example}
% \pan{Apply the terminology of program synthesis to introduce our method.}
%Here, we only provide a high-level description of our planner, and leave more implementation details (e.g., prompts) to later sections.
We formalize our planner as follows:
given the input query $x_0$, the module inventory $\mathcal{M}$, and constraints $\cG$, the natural language planner $\cP$ selects a set of modules that can be executed sequentially to answer the query via generating a program in a natural-language-like format. The module inventory $\mathcal{M}$ consists of a set of pre-built modules: $\{M_i\}$, each corresponding to a tool of various types (Table \ref{tab:tools}). $\cG$ are the constraints for the plan generation, for example, the concurrent relations and sequence orders of modules. In our work, the planner $\cP$ is an LLM prompted to generate a sequence of module names in a few-shot setup. The planner is prompted in natural language with a planning task instruction $\mathcal{I}$, the descriptions of modules in $\mathcal{M}$ with corresponding constraints $\cG$, as well as a few demonstration examples $\mathcal{D}$.  
A $T$-length plan sampled from $\mathcal{P}$ can be denoted as $p = {M^1, \dots, M^T}$, where $M^t$ represents an the $t$-th element in the generated plan and $M^t\in\mathcal{M}$. Formally, given an input query (problem statement) $x_0$, a plan $p$ is generated as follows:
\begin{equation}
    p \leftarrow \cP (x_0; \mathcal{I}, \cM, \cG, \mathcal{D}).
\end{equation}
Given the generated plan, the corresponding modules for each step are then executed sequentially. The plan is a natural-language program where each module is bound simply via string matching. When evaluating the module $M^t$ at time step $t$, the output of the execution $y^t$ is calculated by:
\begin{equation}
 y^t \leftarrow M^t (x^{t-1}; c^{t-1}),
\end{equation}
where $x^{t-1}$ is the input for the current module $M^t$, and $c^{t-1}$ is the cached information (e.g., image semantics, retrieved knowledge, generated programs) resulting from the execution history of modules.
Both the problem input $x^t$ and cache $c^t$ for the next module $M^{t+1}$ are updated, respectively, by:
\begin{equation}
\begin{aligned}
 x^t \leftarrow \texttt{update\_input}(x^{t-1}, y^t), ~~
 c^t \leftarrow \texttt{update\_cache}(c^{t-1}, y^t).
\end{aligned}
\end{equation}

The \texttt{update\_input} and \texttt{update\_cache} functions are hand-designed for each $M_t$. Specifically, \texttt{update\_input} is applied to elements in the input query, including the question, table context, and image. These elements are updated after module execution. \texttt{update\_cache} corresponds to the generation of new information, such as a description for the input image or retrieved knowledge from external resources. Finally, the response $r$ to the query is generated by the last module $M^T$:
\begin{equation}
 r = y^T\leftarrow M^T (x^{T-1}; c^{T-1}).
\end{equation}
% The applications of~\model~are illustrated in Section \ref{sec:application} and see experimental details in Section \ref{app:details} in the appendix.
% The applications of the \model~are detailed in section \ref{sec:application}, and further experimental details can be found in appendix \ref{app:details}.

%, , e.g., OpenAI models, Hugging Face models, GitHub models, search engines, Python interpreters, and rule-based functions.

% \input{codes/algoritm}

\section{Applications of \model}
\label{sec:application}
We demonstrate the applications of \model on two challenging tasks: ScienceQA \cite{lu2022learn} (section \ref{sec:sqa}) and TabMWP \cite{lu2023dynamic} (section \ref{sec:tabmwp}), using the module inventory introduced in section \ref{sec:module}. Further experimental details can be found in appendix \ref{app:details}.

% The module inventory is introduced in section \ref{sec:module}, and the specific designs for these two tasks are presented in section \ref{sec:sqa} and section \ref{sec:tabmwp}, respectively.


\subsection{Module Inventory}
\label{sec:module}

% \pan{Introduce the modular sets. List all the modules}

\begin{wraptable}{r}{0.49\textwidth}
    \centering
    \vspace{-3.7mm}
    \includegraphics[width=0.98\linewidth]{figs/tools.pdf}
    \vspace{-0.8mm}
    \caption{Different tools in our module inventory.}
    \label{tab:tools}
    \vspace{-5mm}
\end{wraptable}

To accommodate various reasoning capabilities over a diverse range of queries, our system utilizes a rich module inventory of various external tools. We provide a high-level overview of this inventory here, with detailed implementations in specific experiments. The complete module inventory, $\mathcal{M}$, is presented in Table \ref{tab:tools}. Each tool within the inventory is defined as follows:
% To accommodate various problem-solving capabilities over a diverse range of problems, it is necessary for our system to leverage a rich module inventory containing various external tools. In this section, we give a high-level description of the module inventory we used and defer the descriptions of detailed implementations to specific experiments.
% The complete module inventory, denoted as $\mathcal{M}$, is presented in Table \ref{tab:tools}. Each tool within the inventory is defined as follows:


\textbf{Knowledge Retrieval} ($M_{kr}$): This module retrieves additional background knowledge crucial for tackling complex problems. It is especially beneficial for specialized domains like science and mathematics, providing context for the task. For example, if a query is about a tax form table, this module could generate knowledge about tax procedures, offering valuable context.
% \textbf{Knowledge Retrieval} ($M_{kr}$): Retrieving extra background knowledge is crucial for assisting the system in tackling complex problems. Here, the ``Knowledge Retrieval'' module is designed to obtain domain-specific knowledge in a generative manner, i.e., prompting the LLMs to generate relevant background information for the given query, as done by \cite{suris2023vipergpt}. Typically, this module is beneficial for providing useful task contexts for solving problems from specialized domains, such as science and mathematics. For instance, if a question is about a tax form table, this module could generate knowledge pertaining to tax procedures, providing valuable context for the task at hand.
% tax regulations and procedures

\textbf{Bing Search} ({$M_{bs}$}): Like ``Knowledge Retrieval'', the ``Bing Search'' module aims to provide wide-ranging task-relevant knowledge. In contrast, it excels when broader or up-to-date information from multiple sources is required. Using the search engine API, this module returns relevant search results based on the input query, which are then parsed and used by subsequent modules to gather richer context information from diverse sources, enhancing problem-solving effectiveness.
% \textbf{Bing Search} ({$M_{bs}$}): Similar to ``Knowledge Retrieval'', the goal of the ``Bing Search'' module is to provide broader coverage of task-relevant knowledge. In contrast to the generative ``Knowledge Retrieval'' module, the ``Bing Search'' module demonstrates its strengths in cases where a broader range of information is needed or the query requires up-to-date information from multiple sources. We implement this module using the search engine API to return relevant search results based on the input query. The returned results can then be parsed and utilized by other modules within the system to gather richer context information from diverse sources to support problem-solving more effectively.


\textbf{Query Generator} ($M_{qg}$): Since the original problem typically lacks a tailored query for retrieving task-relevant information, this module creates search engine queries based on the problem, which are then used by the ``Bing Search'' module. Mostly, it is a good strategy to use the ``Query Generator'' module before the ``Bing Search''. Coupled with the search engine tool, generating more targeted queries generally facilitates both the recall and precision of retrieved information. 
% \textbf{Query Generator} ($M_{qg}$): Generally, the original problem does not contain any tailored query for retrieving task-relevant information from the search engine. Thus, the query generator is designed to create search engine queries based on the given problem, which is then used as inputs to the ``Bing Search'' module. For most cases, it is a good strategy to use the ``Query Generator'' module before the ``Bing Search''. In other words, coupled with the search engine tool, generating more targeted queries generally facilitates both the recall and precision of retrieved information. 


\textbf{Image Captioner} ($M_{ic}$): Designed to generate captions for images, this module provides crucial supplementary context for queries. It is particularly valuable when understanding an image semantically, like identifying objects and interactions in a scene. Using pre-trained models, it translates visual data into language, facilitating effective comprehension and reasoning about image content.
% \textbf{Image Captioner} ($M_{ic}$): This module is designed to generate captions for images, which can be employed to offer additional context for the given question. Typically, the ``Image Captioner'' is utilized when a question requires a semantic understanding of an image. By leveraging pre-trained image captioning models, the ``Image Captioner'' module produces captions for the input image.

\textbf{Text Detector} ($M_{td}$): This module is designed to identify text within a given image. Typically, the ``Text Detector'' is employed when a question requires the extraction of textual information from images containing diagrams, charts, tables, maps, or other visual elements. By effectively detecting text in various formats, this module aids in the analysis and understanding of image-based content.
% and the "has image" field in the metadata is True.


\textbf{Row Lookup} ($M_{rl}$): This module is crucial when queries involve tabular context, as locating relevant cells is often required. Large tables can distract the system, so ``Row Lookup'' simplifies the table by retaining only the rows relevant to the query. If all rows are pertinent, it returns the original table.
% \textbf{Row Lookup} ($M_{rl}$): In situations where questions involve tabular context, locating relevant cells to answer the question is often necessary. Large tables with numerous cells can potentially distract the system when attempting to comprehend the data. The ``Row Lookup'' module addresses this challenge by returning a simplified version of the table, retaining only the rows pertinent to the question. This module accepts a question and a table as input and outputs the simplified table. If all rows are relevant, the original table is returned.

\textbf{Column Lookup} ($M_{cl}$): Like the ``Row Lookup'' module, ``Column Lookup'' addresses questions involving tabular context by focusing on relevant columns. It simplifies the table by retaining only pertinent columns, or returns the original table if all columns are relevant.
% \textbf{Column Lookup} ($M_{cl}$): Similar to the ``Row Lookup'' module, the ``Column Lookup'' module is designed to handle questions involving tabular context by focusing on relevant columns. This module streamlines the table by retaining only the columns that are pertinent to the question. The table keeps the same if all columns are relevant.


\textbf{Table Verbalizer} ($M_{tv}$): Converting structured tables into text is likely to enhance the comprehension of tabular information by various downstream modules as shown by \cite{ma-etal-2022-open} for open-domain question answering, making this module a vital part of our system. It translates tables into easily understandable descriptions for modules like ``Program Generator'' and ``Solution Generator'', particularly useful for small, domain-specific tables like stem-and-leaf plots or function tables. 
% \textbf{Table Verbalizer} ($M_{tv}$): Since the LLM is fundamental to our system, converting structured tables into text is likely to enhance the comprehension of tabular information by various downstream modules as shown by \cite{ma-etal-2022-open} for open-domain question answering. Thus, the module is introduced to convert tables into easily comprehensible descriptions for downstream modules like ``Program Generator'' and ``Solution Generator''. This module is typically employed when the table has a small number of rows and columns and is domain-specific, such as stem-and-leaf plots or function tables. By transforming tabular data into natural language, this module facilitates better understanding and processing by subsequent modules.



\textbf{Program Generator} ($M_{pg}$): Program-aided approaches are shown to enhance the logical and mathematical reasoning abilities of LLMs \cite{wang2022code4struct,gao2022pal,chen2022program,mishra2022lila,imani2023mathprompter,paranjape2023art}. The ``Program Generator'' generates Python programs to solve queries effectively, which is particularly beneficial for queries requiring complex computations or intricate logical operations, such as ``if-else'' statements.
% \textbf{Program Generator} ($M_{pg}$): Recent work has shown that program-aided approaches are able to improve the logical and mathematical reasoning abilities of large language models \cite{wang2022code4struct,gao2022pal,chen2022program,mishra2022lila,imani2023mathprompter,paranjape2023art}. Taking the question and context, the ``Program Generator'' module generates Python programs that can solve the given question effectively. This module is particularly useful when questions and contexts involve complex computations, such as arithmetic operations on multiple numbers, or when questions require intricate logical operations, such as ``if-else'' statements.


\textbf{Program Verifier} ($M_{pv}$): Recent studies highlight the importance of verification to reduce hallucination \cite{peng2023check,madaan2023self}. Hence, ``Program Verifier'' ensures the validity and error-free nature of programs generated by ``Program Generator''. It checks for syntax and logical errors, and potential execution issues, enhancing the reliability and accuracy of the solutions.
% \textbf{Program Verifier} ($M_{pv}$): Recent work emphasizes the contribution of the verifying generation to reduce hallucination \cite{peng2023check,madaan2023self}. Therefore, the ``Program Verifier'' is designed to ensure the validity and error-free nature of the programs generated by the ``Program Generator''. The ``Program Verifier'' checks for syntax errors, logical errors, and other potential issues that may arise during program execution, improving the overall reliability and accuracy of the generated solutions.

\textbf{Program Executor} ($M_{pe}$): This module executes the program generated by ``Program Generator'' and produces the result, bridging the gap between program generation and final solution derivation. 

% \textbf{Solution Generator} ($M_{sg}$): The ``Solution Generator'' module is designed to generate a detailed solution to the input question, considering all the information stored in the cache. This module produces solutions in a chain-of-thought prompting manner, as proposed by \cite{wei2022chain}, ensuring a coherent and well-structured response based on the available information. The planner can rely on this module only if the  planner has high confidence to solve it by itself.

\textbf{Solution Generator} ($M_{sg}$): This module generates a detailed solution to the input query using all the cached information. Employing a chain-of-thought prompting approach~\cite{wei2022chain}, it ensures coherent and well-structured responses. The planner can directly employ this module instead of other functional modules if it can solve the query independently, especially for simpler ones.
% \textbf{Solution Generator} ($M_{sg}$): The ``Solution Generator'' module aims to generate a detailed solution to the input query, taking into account all the information stored in the cache. Employing a chain-of-thought prompting approach \cite{wei2022chain}, this module ensures coherent and well-structured responses based on the available information. The planner relies on this module only if this module is powerful enough to solve the problem independently, especially for simple problems.


\textbf{Answer Generator} ($M_{ag}$): This task-specific module uses a rule-based approach to extract and normalize answers from the results of the ``Program Executor'' or ``Solution Generator''. Unlike the Solution Generator'' that provides detailed multi-step solutions, ``Answer Generator'' serves as the final module in the pipeline, providing concise and task-specific answers.
% \textbf{Answer Generator} ($M_{ag}$): This task-specific module extracts and normalizes the answer from the results generated by the ``Program Executor'' or ``Solution Generator'' using a rule-based approach. In contrast to ``Solution Generator`` that generates detailed multi-step solutions, the ``Answer Generator'' module serves as the final module in the reasoning pipeline, ensuring a concise answer is a task-specific format.


\subsection{Science Question Answering}
\label{sec:sqa}

Science Question Answering (\scienceqa \cite{lu2022learn}) is a diverse benchmark for multi-modal question answering over a range of scientific topics and contexts. As examples illustrated in Figure \ref{fig:showcase_scienceqa}, answering these questions requires various tools and skills like image captioning, text detection, knowledge retrieval, online resource search, and multi-clue visual reasoning. When generating programs for using tools, we limit the search space to the relevant inventory subset (Table \ref{tab:tools_task} in the appendix). Programs are deemed invalid and default to a ``Solution Generator'' and ``Answer Generator'' sequence if these are not the final two elements, following the chain-of-thought prompting baseline \cite{wei2022chain}. See Table \ref{fig:planner_scienceqa} in the appendix for the constructed natural language planner prompt. The prompts for LLM-based modules like Knowledge Retrieval'', ``Query Generator'', and ``Solution Generator'' are shown in Table \ref{fig:planner_scienceqa_kr}, \ref{fig:planner_scienceqa_qg}, and \ref{fig:planner_scienceqa_sg}, respectively, in the appendix.


% When generating programs for using tools, we constrain the search space to the relevant part of the entire inventory, as listed in Table \ref{tab:tools_task} in appendix. 
% Programs are deemed invalid if the modules ``Solution Generator'' and ``Answer Generator'' are not the final two elements. Invalid programs are then set to the default program, consisting of a sequence of ``Solution Generator'' and ``Answer Generator'', which refers to the chain-of-thought prompting baseline \cite{wei2022chain}. 
% The constructed prompt for the natural language planner is displayed in Figure \ref{fig:planner_scienceqa} in appendix. The prompts for LLM-based modules, such as ``Knowledge Retrieval'', ``Query Generator'', and ``Solution Generator'' are  shown in Figure \ref{fig:planner_scienceqa_kr},  Figure \ref{fig:planner_scienceqa_qg}, and Figure \ref{fig:planner_scienceqa_sg} in appendix, respectively.

\subsection{Tabular Mathematical Reasoning}
\label{sec:tabmwp}

\tabmwp \cite{lu2023dynamic} is a mathematical reasoning task involving diverse tabular contexts like schedules, prices, tax forms, plots, and function relations (Figure \ref{fig:showcase_tabmwp}). It requires AI systems to understand various table formats and perform precise numerical or symbolic computations. Like \scienceqa, we constrain the program search space to focus on two tool types: 1) those helping LLMs better digest tabular information (e.g., ``Row Lookup'', ``Column Lookup'',  and ``Table Verbalizer'') and 2) those performing faithful symbolic computations (e.g., ``Program Generator'', ``Program Verifier'', and ``Program Executor'') as listed in Table \ref{tab:tools_task}. The generated programs must meet certain constraints, such as including ``Answer Generator'' and placing ``Program Generator'' prior to both ``Program Verifier'' and ``Program Executor''. Non-compliant programs default to a sequence of ``Program Generator'', ``Program Verifier'', ``Program Executor'', and ``Answer Generator'', aligning with the program-of-thought prompting baseline \cite{chen2022program} with added verification. Non-compliant programs default to a sequence of ``Program Generator'', ``Program Verifier'', ``Program Executor'', and ``Answer Generator'', aligning with the program-of-thought prompting baseline \cite{chen2022program} with added verification.

% \tabmwp \cite{lu2023dynamic} is a mathematical reasoning task on tables. There are diverse tabular contexts, including schedules, prices, tax forms, plots, and function relations. As the examples shown in Figure \ref{fig:showcase_tabmwp}, this task requires AI systems to understand tables of various forms from different domains and perform precise numerical/symbolic computations. Similar to \scienceqa, we again constrain the program search space to focus on two types of tools, particularly, 1) tools can help LLMs better digest tabular information, e.g., ``Row Lookup'', ``Column Lookup'',  and ``Table Verbalizer''; 2) tools can perform faithful symbolic computations, such as ``Program Generator'', ``Program Verifier'', and ``Program Executor''. The full list is shown on the right side of Table \ref{tab:tools_task}. The generated programs adhere to additional constraints, such as the inclusion of ``Answer Generator'', the placement of ``Program Generator'' prior to ``Program Verifier'', and the positioning of ``Program Generator'' before ``Program Executor''. If these conditions are not met, the programs are regarded as invalid and set as a sequence of ``Program Generator'', ``Program Verifier'', ``Program Executor'', and ``Answer Generator''. This program corresponds to the program-of-thought prompting baseline \cite{chen2022program} with added program verification.


%\newpage
\section{Experiments}
\label{sec:experiment}

We assess our \model's effectiveness and adaptability on two complex reasoning tasks, \scienceqa~\cite{lu2022learn} and \tabmwp~\cite{lu2023dynamic}. See experimental details  in appendix \ref{app:details} in the appendix.

% We conduct experiments on two complex reasoning tasks, \scienceqa \cite{lu2022learn} and \tabmwp \cite{lu2023dynamic}, to evaluate our \model in terms of effectiveness and adaptability. The experimental details are introduced in appendix \ref{app:details} in the appendix.



\subsection{Experimental Results}

% Table
\input{tables/results_scienceqa}




\textbf{\scienceqa.} Table \ref{tab:scienceqa} presents the results of existing baselines and our \model, with key results highlighted in Figure \ref{fig:results_highlight} (a). Employing ChatGPT \cite{openai2022chatgpt} as the base LLM, \model achieves a 79.93\% accuracy, a 1.62\% improvement over Chain-of-Thought (CoT) \cite{wei2022chain} prompted ChatGPT. Notably, \model is a generalized form of CoT, where the generated program is a sequence of ``Solution Generator'' and ``Answer Generator''. \model benefits from additional tool usage, such as ``Knowledge Retrieval'', ``Bing Search'', ``Image Captioner'', and ``Text Detector''. When built upon GPT-4 \cite{OpenAI2023GPT4TR}, our model attains an accuracy of 86.54\%, outperforming GPT-4 CoT \cite{lu2022learn} by 2.55\% and GPT-3 CoT by 11.37\%, creating the new state of the art in few-shot settings.

% \pan{Analyze the accuracy scores with different settings: enabled/disabled some modules, accuracy among different groups of a number of table cells, accuracy for questions with/without the text in the image, and so on.}

% Table
\input{tables/results_tabmwp}

\begin{figure*}[t!] 
  \begin{minipage}{0.50\textwidth} 
    \centering
    \includegraphics[width=1.0\textwidth]{figs/scienceqa_bar.pdf}
    \caption*{(a) Results on \scienceqa}
    \label{results_highlight_scienceqa}
  \end{minipage}
  \hfill
  \begin{minipage}{0.50\textwidth} 
    \centering
    \includegraphics[width=1.0\textwidth]{figs/tabmwp_bar.pdf}
    \caption*{(b) Results on \tabmwp} 
    \label{results_highlight_tabmwp}
  \end{minipage}
  \caption{Results of main baselines and \model. Dashed lines represent human performance.
  % on \scienceqa and \tabmwp. The vertical dashed line represents human performance. 
  % On \scienceqa, \model using GPT-4 surpasses the previously published best few-shot model and attains results comparable to fine-tuned models. On \tabmwp, \model with GPT-4 achieves state-of-the-art results, exceeding human performance by 8.6\%.
  }
  \vspace{-3mm}
  \label{fig:results_highlight}
\end{figure*}

% \pan{Specialize the selection and implementation of modules }

\textbf{\tabmwp.} Table \ref{tab:tabmwp} presents results with key models in Figure \ref{fig:results_highlight} (b). Similarly, significant improvements are observed for \model over both fine-tuned and few-shot models. It is worth noting that both CoT and Program-of-Thought (PoT) \cite{chen2022program} can be viewed as special cases of \model. Apart from ``Solution Generator'' and ``Answer Generator'', CoT doesn't utilize any tool, while PoT only relies on symbolic programming tools like ``Program Generator'' and ``Program Executor''. \model (ChatGPT) outperforms ChatGPT CoT and ChatGPT PoT by 11.25\% and 3.79\%, respectively, emphasizing our enriched tool set's advantage. With GPT-4, \model gains an additional 5.50\%, reaching a 98.78\% accuracy. Notably, \model (GPT-4) surpasses Codex PoT-SC \cite{chen2022program}, the best-published model, by 17.0\% and human performance by 8.56\%.

% CoT does not use any tool whereas PoT only resorts to symbolic programming tools in our inventory, e.g., ``Program Generator'', ``Program Executor'', and ``Answer Generator''. \model (ChatGPT) achieves improvements of 11.25\% and 3.79\% over ChatGPT CoT and ChatGPT PoT, respectively, demonstrating the advantage of our enriched tool set. By updating the underlying LLM with GPT-4, our \model achieves a further gain of 5.50\%, resulting in a 98.78\% accuracy. Remarkably, our \model (GPT-4) not only surpasses the previous best-performing model (Codex PoT-SC \cite{chen2022program}) by 17.0\%, but also outperforms the human performance by 8.56\%.

\subsection{Qualitative Analysis}




\paragraph{Tool use planning.} The proportions of key tools called in the programs from \model on \scienceqa and \tabmwp are visualized in Figure \ref{fig:tool_call_scienceqa} and Figure \ref{fig:tool_call_tabmwp} (in the appendix), respectively. Interestingly, ChatGPT and GPT-4 exhibit different planning behaviors. Generally, ChatGPT has a strong bias toward using or not using certain tools,  highly influenced by in-context examples. For instance, ChatGPT calls ``Knowledge Retrieval'' in 72\% of queries but only calls ``Bing Search'' in 3\% of cases on \scienceqa; on TabMWP, ChatGPT heavily relies on ``Row Lookup'' (47\%) but calls ``Column Lookup'' less frequently (4\%). However, GPT-4 acts more \textit{objectively} and \textit{rationally} in tool selection. For example, GPT-4 calls ``Knowledge Retrieval'' more frequently (81\% vs. 72\%) and calls ``Bing Search'' more than ChatGPT (11\% vs. 3\%) when answering scientific questions on \scienceqa. Impressively, GPT-4 consistently calls ``Query Generator'' and ``Bing Search'' simultaneously by observing the tool usage descriptions, while ChatGPT lacks such reasoning capability.
% However, GPT-4 acts more \textit{objectively} and \textit{rationally} when determining which tool to use or not. 
% We visualize the proportions of key tools called and not called in the generated programs from \model (ChatGPT) and \model (GPT-4) on \scienceqa (shown in Figure \ref{fig:tool_call_scienceqa}) and on \tabmwp (shown in Figure \ref{fig:tool_call_tabmwp} in the appendix), respectively. 

\begin{figure*}[t!]
    \centering
    % \vspace{-3mm}
    \includegraphics[width=1.0\linewidth]{figs/tool_call_bar_scienceqa.pdf}
    % \vspace{-3mm}
    \caption{Tools called in the generated programs from \model on \scienceqa.}
    % \vspace{-3mm}
    \label{fig:tool_call_scienceqa}
\end{figure*}

\begin{wraptable}{r}{0.41\textwidth}
 \vspace{-4mm}
 \renewcommand\tabcolsep{1.0pt} % column space
 \renewcommand\arraystretch{1.0} % row space
 \resizebox{1.0\linewidth}{!}{
 \begin{tabular}{lcc} 
 \toprule
 Module & $\Delta$ (\scienceqa) & $\Delta$ (\tabmwp) \\
 \midrule
 Knowledge Retrieval & -7.8\% & -2.2\% \\
 Bing Search & -7.4\% & - \\
 Text Detector & -8.4\% & - \\
 Image Captioner & -6.0\% & - \\
 Program Generator & - & -7.4\% \\
 Table Verbalizer & - & -0.2\% \\
 \bottomrule
 \end{tabular}
 }
 \vspace{-1mm}
 \caption{\small{Score drop with disabled modules.}}
 \label{tab:disabled_module}
 \vspace{-3mm}
\end{wraptable}


\paragraph{Ablation study with disabled modules.} We study the accuracy decline of \model when key modules in the generated programs are disabled (Table \ref{tab:disabled_module}), using ChaptGPT as the underlying LLMs and 500 test examples. The results reveal that ``Knowledge Retrieval'' plays a vital role in both tasks. Domain-specific tools, such as the search engine and vision models for \scienceqa, and program tools for \tabmwp, also prove to be important.

\paragraph{Module transitions.} We visualize the transition graphs of modules for generated programs by \model (GPT-4) on \scienceqa and \tabmwp in Figure \ref{fig:transition_scienceqa} and \ref{fig:transition_tabmwp}, respectively.
The transition probabilities in these graphs are computed from the tool transitions observed on the test sets. These graphs illustrate that the GPT-4 planner is able to make good decisions on how to sequence tools in a few-shot setup. For example on ScienceQA, \model often decides to rely on either  ``Knowledge Retriever'' or ``Bing Search'', but rarely both. On TabMWP, we observe two main modes: either going through the solution-executor module or via the program verifier and executor.  
% of these two datasets

% \include{tables/tool_num}

\subsection{Case Study} 
\paragraph{Visualization examples.} 

Three examples from \model (GPT-4) on \scienceqa are visualized in Figure \ref{fig:showcase_scienceqa}. \model (GPT-4) is able to adapt to different input queries by generating programs that compose various tools and executing them sequentially to obtain accurate responses. For instance, to answer the first question, \textit{What is the direction of this push?}, the system calls the image captioner model to extract semantic information from the image and employs the knowledge retrieval model to gather background knowledge for multi-modal reasoning. In the second example, the natural language planner infers that a text detector tool is needed to understand the context of the ad. The third query (more details provided in Figure \ref{fig:showcase_scienceqa_more} in the appendix), \textit{Which animal's skin is adapted for survival in cold places?}, involves scientific terminology related to animal survival. The planner decides to call the Bing search engine to access domain-specific knowledge, benefiting from the numerous online resources. Discussions on examples on \tabmwp are provided in the appendix \ref{app:results}.
% In the third example (with more details provided in Figure \ref{fig:showcase_scienceqa_more} in the appendix), the query asks, \textit{Which animal's skin is adapted for survival in cold places?}, which involves scientific terminology related to animal survival. Consequently, the planner decides to rely on the Bing search engine for domain-specific knowledge, benefiting from the numerous online resources available. 


\noindent\textbf{Failure cases and limitations.} Examples of failure cases from \model (GPT-4) are illustrated in the appendix. Inaccurate responses may arise from the limitations of the current modules or from suboptimal programs generated by the planner. Additionally, the module inventory may lack tools capable of addressing specific abilities. Future directions could involve upgrading the modules and the planner, or expanding the module inventory to support a broader range of capabilities. Further limitations and broader impacts are respectively discussed in sections \ref{app:limitations} and \ref{app:impacts} of the appendix.


% The examples of failure cases by \model (GPT-4) are visualized in the appendix. The inaccurate response could be due to the limitations of modules in the current limitations (Tables \ref{fig:failure_scienceqa_1}, \ref{fig:failure_scienceqa_2}, \ref{fig:failure_tabmwp_1}, \ref{fig:failure_tabmwp_3}). The error can also result from the suboptimal programs from the planner (Tables \ref{fig:failure_scienceqa_2}, \ref{fig:failure_tabmwp_2}, \ref{fig:failure_tabmwp_3}) or the module inventory lacking tools that are capable of addressing specific abilities (Tables \ref{fig:failure_scienceqa_3}, \ref{fig:failure_tabmwp_3}). The future directions can upgrade the modules and the planner, or scale up the module inventory to support more diverse capabilities.


% \pan{Analyze the accuracy scores with different settings: enabled/disabled some modules, accuracy among different groups of a number of table cells, accuracy for questions with/without the text in the image, and so on.}

% \subsection{Case Study: XXX}

% \pan{Add one demo from the team.}

% \subsection{Case Study: XXX}

% \pan{Add one more demo from the team.}

%\newpage
% \section{Future Work}
% \label{sec:future}


%\newpage
\section{Conclusion}
\label{sec:conclusion}


In conclusion, we introduce a novel \textit{plug-and-play compositional} reasoning framework, \model, that addresses the limitations of current large language models by augmenting them with external tools in a plug-and-play manner. Our approach employs a diverse set of tools and demonstrates impressive adaptability and effectiveness on two challenging benchmarks, \scienceqa and \tabmwp. By achieving significant improvements in accuracy over existing state-of-the-art models, \model showcases its potential for addressing real-world queries across various domains. 

% \pan{future work, discuss the self-programming idea?} 



%%%%%%%%% Acknowledgment
% \clearpage
\section{Acknowledgment}
We would like to thank Chunyuan Li, Qiuyuan Huang, and other members of the Deep Learning group at Microsoft Research for their valuable discussions. We also thank Fan Yin from University of California, Los Angeles, and Mingyang Sun from University of Electronic Science and Technology of China for their thorough review of our paper and constructive feedback.

% Yang Sun: the University of Electronic Science and Technology of China

% Fan Yin for constructive comments.

%%%%%%%%% REFERENCES
% \clearpage
\bibliographystyle{plain} 
{
\small
\bibliography{egbib}
% \nocite{*}
}



==> v2_arxiv_backup/tool.tex <==
\begin{table*}[t]
\centering
% \footnotesize
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{llll}
\toprule
\textbf{Task} & \textbf{Math category} & \textbf{IID} & \textbf{OOD} \\
\midrule
\multirow{7}{*}{\textsc{Task 1}} & \multirow{7}{*}{Basic math}
& \texttt{addsub.json} & \texttt{MCTaco\_event\_duration\_structured.json} \\
& & \texttt{Numersense\_structured.json} & \texttt{NumGLUE\_Task3.json}  \\
& & \texttt{MCTaco\_stationarity\_structured.json} & \\
& & \texttt{MCTaco\_frequency\_structured.json} & \\
& & \texttt{MCTaco\_event\_typical\_time\_structured.json} & \\
& & \texttt{MCTaco\_event\_ordering\_structured.json} & \\
& & \texttt{NumGLUE\_Task7.json} & \\
\midrule
\multirow{7}{*}{\textsc{Task 2}} & \multirow{7}{*}{Muldiv}
& \texttt{singleop.json} & \texttt{svamp\_structured.json} \\
& & \texttt{multiarith.json} & \texttt{NumGLUE\_Task4.json} \\
& & \texttt{asdiv.json} & \texttt{} \\
& & \texttt{GSM8k\_structured.json} & \texttt{} \\
& & \texttt{NumGLUE\_Task1.json} & \texttt{} \\
& & \texttt{NumGLUE\_Task2.json} & \texttt{} \\
& & \texttt{deepmind\_mathematics\_muldiv.json} & \texttt{} \\
\midrule
\multirow{8}{*}{\textsc{Task 8}} & \multirow{8}{*}{Number theory}
& \texttt{mathqa\_physics.json} & \texttt{mbpp\_structured.json} \\
& & \texttt{APPS\_structured.json} & \texttt{mathqa\_other.json} \\
& & \texttt{mathqa\_gain.json} & \texttt{} \\
& & \texttt{amps\_number\_theory.json} & \texttt{} \\
& & \texttt{mathqa\_general.json} & \texttt{} \\
& & \texttt{conala\_structured.json} & \texttt{} \\
& & \texttt{NumGLUE\_Task5.json} & \texttt{} \\
& & \texttt{deepmind\_mathematics\_numbertheory.json} & \texttt{} \\
\midrule
\multirow{5}{*}{\textsc{Task 4}} & \multirow{5}{*}{Algebra}
& \texttt{singleq.json} & \texttt{draw\_structured.json} \\
& & \texttt{simuleq.json} & \texttt{dolphin\_structured.json} \\
& & \texttt{amps\_algebra.json} & \texttt{} \\
& & \texttt{NumGLUE\_Task8.json} & \texttt{} \\
& & \texttt{deepmind\_mathematics\_algebra.json} & \texttt{} \\
\midrule
\multirow{1}{*}{\textsc{Task 5}} & \multirow{1}{*}{Geometry}
& \texttt{amps\_geometry.json} & \texttt{mathqa\_geometry.json} \\
\midrule
\multirow{1}{*}{\textsc{Task 6}} & \multirow{1}{*}{Statistics} 
& \texttt{amps\_counting\_and\_stats.json} & \texttt{mathqa\_probability.json} \\
\midrule
\multirow{2}{*}{\textsc{Task 7}} & \multirow{2}{*}{Calculus}
& \texttt{amps\_calculus.json} & \texttt{deepmind\_mathematics\_calculus.json} \\
& & \texttt{deepmind\_mathematics\_basicmath.json} & \texttt{} \\
\midrule
\multirow{1}{*}{\textsc{Task 8}} & \multirow{1}{*}{Linear algebra}
& \texttt{amps\_linear\_algebra.json} & \texttt{} \\
\midrule
\multirow{1}{*}{\textsc{Task 9}} & \multirow{1}{*}{Advanced math}
& \texttt{MATH\_crowdsourced.json} & \texttt{} \\
\bottomrule
\end{tabular}
}
\caption{Raw datasets used to create different tasks in \lila across different math categories.}
\label{tab:tools}
\end{table*}
